Quorum Subsumption for Heterogeneous Quorum Systems

Byzantine quorum systems provide higher throughput than proof-of-work and incur modest energy consumption. Further, their modern incarnations incorporate personalized and heterogeneous trust. Thus, they are emerging as an appealing candidate for global financial infrastructure. However, since their quorums are not uniform across processes anymore, the properties that they should maintain to support abstractions such as reliable broadcast and consensus are not well-understood. It has been shown that the two properties quorum intersection and availability are necessary. In this paper, we prove that they are not sufficient. We then define the notion of quorum subsumption, and show that the three conditions together are sufficient: we present reliable broadcast and consensus protocols, and prove their correctness for quorum systems that provide the three properties.

==> BRBIntegrity.tex <==
\begin{lemma}
   The BRB protocol guarantees integrity.
%     for all the well-behaved processes.
\end{lemma}

\begin{proof}
    We assume that a well-behaved process $p$ delivers a message $m$ from a well-behaved sender process $p'$,
    and prove that the process $p'$ has broadcast $m$.     
    We first prove that 
    a well-behaved process has received echo messages from at least one of its quorums.

    Since the well-behaved process $p$ delivered $m$, 
    it has received a quorum $q_p$ of ready messages.
    By the strong availability assumption, 
    $P$ is non-empty; therefore,
%     \ec{This is only true if $P$ is non-empty, which is strange since integrity is not qualified by $P$. 
%     Also, $P$ can technically be empty for all the other properties.
%     Maybe something about non-trivial?
%     }
    there exists a process 
%     $p$ 
    with a quorum $q$ that is well-behaved and quorum subsuming.
%     
    By quorum intersection, 
%     $q \cap q_r \cap \W \neq \emptyset$.
    $q_p$ and $q$ intersect at a well-behaved process $p_i$.
%     Let $p_i$ be a member of $q \cap q_r \cap \W$ which sent the ready message.
    The process $p_i$ sent a ready message (that $p$ received).
    The well-behaved process $p_i$ sends a ready message only if it
    either (1) receives echo messages from a quorum of $p_i$, 
    or (2) receives ready messages from a $p_i$-blocking set $B$.
%
    The first case is immediately the conclusion with the process $p_i$.
%
    Let us consider the second case.
    By quorum subsumption, 
    since $p_i$ is in $q$, 
    $p_i$ has a quorum $q_i$ that is a subset of $q$.
%
    Since $B$ is a blocking set of $p_i$,
    $B$ intersects with $q_i$.
    Therefore, $B$ intersects with $q$.
%     $\exists q_i \in \Q(p_i), q_i \subseteq q \subseteq \W \wedge b \cap q_i \neq \emptyset$.  
   The processes in $B$ sent ready messages.
   Thus, there are processes in $q$ that sent ready messages.
   Let $p_f$ be the first process in $q$ that sent a ready message.
   All members of $q$ are well-behaved.
% 
    A well-behaved process $p_f$ sends a ready message only if it
    either (1) receives echo messages from a quorum of $p_f$, 
    or (2) receives ready messages from a $p_f$-blocking set $B'$.
    The first case is immediately the conclusion with the process $p_f$.
    Let us consider the second case.   
    Applying the same reasoning as for $p_i$ to $p_f$
    derives that $B'$ intersects with $q$.
%
    Thus, $p_f$ has received a ready message from a process in $q$.
    Therefore, $p_f$ is not the first process in $q$ to send a ready message.
    This is a contradiction with the definition of $p_f$ above.


    We now use the fact that 
    a well-behaved process has received echo messages from at least one of its quorums.
%
   By quorum intersection at well-behaved processes,
   every quorum of a well-behaved process includes a well-behaved process.
   %Then the first ready message is sent by receiving a quorum of echo messages.
%    Since every quorum of a well-behaved process includes itself,    
%    $q_e$ includes $p_e$.
%     
%     Therefore, $p_e$ has received an echo message from itself.
   Thus, a well-behaved process $p_w$ has sent an echo message.
    A well-behaved process sends an echo message only after receiving it from the sender $p'$.
%     
    Since the sender $p'$ is well-behaved,
    and $p_w$ has received the message $m$ from it,
    by the integrity of point-to-point links,
    $p'$ has previously sent $m$ to $p_w$.
    Since $p'$ is well-behaved, 
    it has sent $m$ to every process.
%
%     \ec{
%     Suppose a well-behaved process $r$ delivers a message $m$ and the sender is well-behaved, 
%     but the sender did not previously broadcast $m$, towards contradiction.
%     If $r$ delivers $m$, then it received a quorum $q_r$ of consistent ready messages.
%     }
%     
%     \ec{
%     Let $p \in P$.
%     Let $q_p$ be the complete quorum of $p$.
%     By quorum intersection, there is a well-behaved process $p_i \in q_p \cap q_r$.
%     If $p_i$ sent a ready message to $r$,
%     then one of the following must be true:
%     (1) $p_i$ received a quorum of consistent echo messages, or
%     (2) $p_i$ received a $p_i$-blocking set of consistent ready messages.
%     }
% 
%     \ec{
%     In the first case, 
%     since every quorum of $p_i$ contains itself,
%     $p_i$ sent an echo message (to itself).
%     However, a well-behaved process only sends an echo message upon receiving a message from the sender,
%     contradicting the assumption that the sender did not broadcast $m$.
%     }
% 
%     \ec{
%     In the second case,
%     $p_i$ received a $p_i$-blocking set of consistent ready messages.
%     (Can you just do $p_f$ here as well?)
%     }
\end{proof}


==> BRBTotality.tex <==
%\textbf{Totality}
\begin{lemma}
%     If the quorum system $\Q$ is available for $P$, then 
    The BRB protocol guarantees totality for $P$.
\end{lemma}

\begin{proof}
    We assume that a well-behaved process $p$ has delivered $m$, 
    and show that every well-behaved process $p' ∈ P$ delivers $m$.
%     
    We first show that every well-behaved process $p''$ sends ready messages for $m$
    to its followers.

    The well-behaved process $p$ delivers $m$ only when 
    it receives a quorum $q$ of ready messages for $m$.
%
%     \cap \W
%     $\forall p' \in \W, \forall q' \in \Q(p'), q \cap q' \cap \W \neq \emptyset$.
% 
    Consider a quorum $q''_i$ of $p''$.
    By quorum intersection, $q$ and $q''_i$ intersect in at least a well-behaved process $p_i$.
%     Let $I_i$ be the intersection of the well-behaved processes of $q$,
%     and $q''_i$.
%     Consider an arbitrary process $p_i$ in $I_i$.
%     By quorum intersection,
%     $q$ and $q''$ intersect at a well-behaved process $p_i$.
%     Consider a process $p_i$ in the intersection of well-behaved processes of $q$, and $q''$.
    Since $p_i$ is in $q''_i$, 
%     then $p''$ is a follower of $p_i$.
    then $p_i$ has $p''$ as a follower.
%
%     All well-behaved processes in $q$ send ready messages to their followers including $p''$.
%     All well-behaved processes in $q$ send ready messages to their followers.
%     Thus, $p_i$ sends a ready message to $p''$.
%     Thus, $p_i$ sends a ready message to $p''$.
%
    Let $I$ be the union of the processes $p_i$ for all quorums $q''_i$ of $p''$.
    By construction,
    the set of processes $I$ are a subset of $q$, a blocking set of $p''$, and have $p''$ as a follower.
%     $p''$ is a follower of it.
%     
%     By quorum intersection,
%     $q$ intersects all quorums in the system in at least one well-behaved process.
%
%     Therefore, 
% %     for any well-behaved process $p'$, 
%     well-behaved processes of $q$ are $p''$-blocking.
% 
%    Since all processes in $q$ have broadcast ready messages,
   All well-behaved processes in $q$ send ready messages to their followers.
   Thus, the set of processes $I$ send ready messages to $p''$.
%
   Thus, $p''$ receives a blocking set of ready messages,
   and sends ready messages to its followers.
%     The well-behaved process $p'$ has a quorum $q'$ with all well-behaved members.


   Thus, every well-behaved process $p''$ sends ready messages to their followers.
   By weak availability, $p' \in P$ has a quorum $q'$ with all well-behaved members.   
   Thus, the process $p'$ will receive ready messages from $q'$, and delivers $m$.
% 
%     \ml{Eric, the following proof looks good. It is just that direct proofs are more natural than proofs by contradiction. I took parts of the proof below to the direct proof above.}
% 
%     \ec{
%     Suppose a well-behaved process $r$ delivers a message, 
%     but there is some process $p \in P$ that does not deliver a message, towards contradiction.
%     Since the quorum system is strongly available for $P$, and $p \in P$,
%     $p$ has at least one complete quorum $q_p$.
%     If $p$ does not deliver a message, it never receives any quorum of consistent ready messages.
%     This means at least one process in $q_p$ does not send a ready message to $p$.
%     Let this process be $p'$.
%     If (well-behaved) $p'$ does not send a ready message to $p$,
%     it did not receive a blocking set of consistent ready messages (nor a quorum of consistent echo messages).
%     }
%     
%     \ec{
%     Since $r$ delivers a message,
%     it must have received a quorum $q_r$ of consistent ready messages.
%     By quorum intersection, for every quorum of $p'$, it intersects $q_r$ at at least one well-behaved process.
%     That is, $q_r \cap \W$ is a blocking set for $p'$.
%     Then, if every well-behaved process in $q_r$ sent a ready message to $r$, then it must also have sent a ready message to $p'$.
%     However, this means $p'$ would have received a blocking set of consistent ready messages,
%     thus reaching a contradiction.
%     }    
\end{proof}


==> ConsensusTermination.tex <==
%\textbf{Weak liveness}
\begin{lemma}[Termination]
% If the quorum system $\Q$ is strongly available for $P$, then 
The consensus protocol guarantees termination for $P$.
\end{lemma}




\begin{proof}
The proof will refer to the notions of locked for federated voting.
We first visit these notions, and then describe the proof of termination.


We saw in the explanation of the protocol that
there are executions that Byzantine processes can lock a federated voting instance
for a certain value (such as commit).
Let us remember that example.
Consider that we have 4 processes, one of them is Byzantine,
and any set of 3 processes is a quorum.
Let the Byzantine process send a message $m$ to one well-behaved process.
That well-behaved process echos $m$.
% However, a well-behaved process has already echoed commit,
If the Byzantine process remains silent,
the remaining 2 well-behaved processes are not a quorum,
and even if both echo another message $m'$,
they cannot make the federated voting deliver $m'$.
% 
This execution is shown in the first two rounds of messages in \autoref{fig:proof-fig}.
% 
In this execution, the federated voting instance of $b$ is locked for $m = \mathbb{C}$ by $l₁$ and $p₃$,
and
although $l₂$ and $p₄$ try to make it deliver $m' = \mathbb{A}$, it does not.
%  
However, if the Byzantine process echos $m'$ as well,
then they form a quorum, and can make $m'$ be delivered.
%  
Well-behaved processes alone cannot make the instance deliver a different value,
but well-behaved and Byzantine processes together can.
We call these states of the federated voting abstraction soft-locked.



We note that 
there are also states of a federated voting instance where
even if well-behaved and Byzantine processes 
work together, they cannot make the instance deliver a different value.
We call them hard-locked.
% We first note that
% after certain steps,
% a federated voting instance can get locked for a certain value.
%
As above,
% consider an execution of federated voting where 
% a blocking set of a process $p$ in $P$ echos a message $m$.
% The process $p$ cannot deliver any message other than $m$.
% If 
consider an execution with 4 processes,
% and a Byzantine sender,
and quorums of size 3.
% 
Let a Byzantine process send $m$ to two well-behaved processes, and make them echo $m$.
% sender sends the message $m$ to two of the process and they 
By the protocol,
in order to deliver a message, a process needs to receive at least three ready messages.
Further,
in order to send a ready message, a process needs to receive
at least either
three echo messages
or
two ready messages.
% 
Therefore, to deliver any other message $m'$, 
at least 3 processes should echo $m'$.
Since 2 well-behaved processes out of 4 processes already echoed $m$, and
well-behaved processes echo only once,
there are not 3 processes to echo $m'$,
and make it delivered.
% the message $m'$ cannot be delivered.
% 
The federated voting abstraction is hard-locked for $m$.


% a well-behaved process 
% For example, 
% as we saw in the proof of consistency of BRB,
% a process can deliver a message $m$ if 
% then no well-behaved process $p'$ can deliver another message $m'$.
% This is because
% the fact that $p$ sent ready $m$
% can be tracked back to 
% the fact that some well-behaved process received echo message from one of its quorums $q$.
% Because of quorum intersection,
% a well-behaved process $p$ sends ready messages for $m$,


We now consider the proof of termination.
By the eventual leader election,
there will eventually be a well-behaved leader with a long enough timeout.
Let $b$ be the $\candidate$ ballot of the leader.
% 
The leader tries to abort all ballots lower and incompatible with $b$
at
\autoref{algC:leader-abort}
and
\autoref{algC:abort-new-round}.
We consider three cases based on whether
there is a ballot $b' ⋦ b$ that
% $ below and incompatible with $
% is either committed or is locked for commit.
is locked for commit.
% (We say that a ballot is committed if a well-behaved process has delivered commit for that ballot.)


Case 1:
There is no such ballot $b'$.
The leader can abort all ballots below and incompatible with $b$
at \autoref{algC:prepared},
and broadcast commit for $b$
at \autoref{algC:leader-commit}.
By the validity of federated voting,
all processes in $P$ eventually deliver commit for $b$
at \autoref{algC:commit-prepared},
and decide its value
at \autoref{algC:decision-reponse}.



Case 2:
There is such a ballot $b'$ that is soft-locked for commit.
% but 
% Byzantine and well-behaved processes together can make the instance deliver abort.
%
In order to prepare $b$,
the leader tries to abort $b'$.
If the Byzantine processes cooperate,
it can abort $b'$ and prepare $b$
at \autoref{algC:prepared}, 
and broadcast commit for $b$
at \autoref{algC:leader-commit}.
% 
However, if the Byzantine processes do not cooperate,
the leader cannot abort $b'$.
Therefore, the leader does not succeed, and the timeout is triggered.
Eventually, a well-behaved process $l$ will be the leader.
% 
Since the delay $Δ$ is larger than the bounded communication delay after GST,
% The delay $Δ$ for the leader $l'$ helps him to observe the highest prepared ballot $b$,
the leader $l$ observes the highest prepared ballot $b$
at \autoref{algC:prepared},
and adopts its value as the value of its $\candidate$ $b'$
at \autoref{algC:prepare-candidate}.
We note that when it tries to prepare $b'$, 
since $b'$ is compatible with $b$, it does not need to abort $b$.
Therefore, it can prepare and broadcast commit for $b'$
at \autoref{algC:leader-commit}.
% and decide.
By the validity of federated voting,
all processes in $P$ eventually deliver commit for $b'$
at \autoref{algC:commit-prepared},
and decide its value
at \autoref{algC:decision-reponse}.



Case 3:
There is such a ballot $b'$ that is hard-locked for commit.
% but 
% even Byzantine and well-behaved processes together cannot make the instance deliver abort.
% 
% By the consistency of federated voting, 
Ballot $b'$ cannot be aborted.
Therefore,
% no well-behaved leader 
no well-behaved process can prepare 
% and try to commit 
a ballot with a value incompatible with $b'$.
The current leader will eventually timeout.
% 
Further, all ballots $b'' ⋦ b'$ should have been aborted
since processes accept commit for $b'$ only if $b'$ is $\prepared$
at \autoref{algC:commit-prepared}.
%
By the totality of federated voting,
eventually a well-behaved leader that has delivered abort for all ballots $b''$
% below and incompatible with $b'$
will be elected.
Therefore, that leader finds $b'$ prepared
at \autoref{algC:prepared}-\ref{algC:update-prepared}, and 
adopts its value as the value of its $\candidate$ ballot $b₂''$
at \autoref{algC:update-candidate}.
Thus, $b₂''$ is compatible with $b'$.
%
As we saw above,
% any prepared ballot larger than $b'$ is compatible with $b'$
no ballot incompatible with $b'$ can be prepared.
Thus, no ballot incompatible with $b₂''$ can be prepared.
% The candidate of that leader
Thus, the leader can successfully prepare $b₂''$ 
at \autoref{algC:prepared}, 
and broadcast commit for $b₂''$
at \autoref{algC:leader-commit}-\ref{algC:prepare-candidate}.
By the validity of federated voting,
all processes in $P$ eventually deliver commit for $b₂''$
at \autoref{algC:commit-prepared},
and decide its value
at \autoref{algC:decision-reponse}.
% 
\end{proof}








==> FullRelatedWork.tex <==
% \section{Related Works}
\section{Related Works and Discussion}

% \subsection{Heterogeneous Quorum Systems}
% \subsection{Quorum Systems with Non-uniform Trust}
% \subsection{\textbf{Quorum Systems with Decentralized Trust}}
% \textbf{∗Quorum Systems with Decentralized Trust. \ }
\textbf{∗Quorum Systems with Heterogeneous Trust. \ }
% 
The blockchain technology raised the interest in quorum systems
% heterogeneous
that 
% support open
% admission and release of participants,
% is decentralized,
% and
% the participants are dynamic,
% membership
% the trust preferences of participants are not uniform and are not globally known.
allow the trust preferences of participants to be non-uniform.
% and are not globally known.
% 
Ripple \cite{schwartz2014ripple} and
Cobalt \cite{macbrough2018cobalt}
pioneered decentralized trust.
They let each node specify a list, called the unique node list (UNL), of processes that it trusts.
% and provide atomic broadcast.
% with probabilistic liveness.
However, they assume that 60-90\% of two such lists overlap for quorum intersection,
but do not consider quorum availability or sharing.
%Violation of this assumption can compromise the security of the network
%\cite{amores2020security}.



Stellar \cite{mazieres2015stellar,lokhava2019fast}
provides a consensus protocol for
federated Byzantine quorum systems 
%\cite{garcia2018federated,garcia2019deconstructing}
where
nodes are allowed to specify sets of processes, called slices,
that they trust.
% The Stellar system \cite{lokhava2019fast} uses hierarchies and thresholds to specify slices.
% 
A process finds a quorum
% derived 
starting from a slice 
by iteratively probing processes in the current set, 
and adding their slices to the set.
% and provides an agreement protocol.
However,
% the decentralized calculation of quorums 
since each process calculates its own quorums separately,
to make sure that the resulting quorums intersect,
quorums have to comply with certain hierarchies and thresholds.
% 
Follow-up research analyzed the decentralization 
% extent 
of FBQS systems
\cite{bracciali2021decentralization,florian2022sum}.
% 
% Therefore, they provide limited decentralization
% \cite{bracciali2021decentralization,florian2022sum}.
% 
% the resulting quorums do not necessarily intersect.
% this 
% % decentralized 
% calculation by different processes
% % two 
% does not guarantee intersection for their quorums.
% The decentralized calculation of 
% Quorums that are do not guarantee their intersection.
%\xl{Do we still need this?}Therefore, to prevent forks, a global intersection check is continually executed over the network.
% 
Federated Byzantine quorum systems (FBQS) \cite{garcia2018federated,garcia2019deconstructing} formally models Stellar, 
and presents reliable broadcast and consensus protocols, and their correctness proofs.
% 
In comparison,
the assumptions of the protocols presented in this paper are weaker, and their guarantees are stronger.
% 
The FBQS model is based a subset of processes called the intact set.
The intact set is a subset of processes that have strong availability, 
that is in turn, a subset of processes that have weak availability.
In FBQS, the intersections of quorums should have a process in the intact set;
however, in HQS, they only need to have a well-behaved process.
% 
The validity and totality properties for the reliable broadcast for FBQS are restricted to 
the intact set.
% The guarantees of FBQS involves on a set of processes called the intact set.
On the other hand,
%
% Totality: FBQS for intact. HQS: weakly available
% Validity: FBQS for intact. HQS: strongly available
the reliable broadcast protocol in this paper provides
%
% Our conditions are strictly weaker: only well-behaved quorum intersection is enough.
totality for all processes that have weak availability, 
and
validity for all processes that have strong availability.
% 
Further
the abstract consensus protocol for FBQS 
does not provide weak validity,
and 
provides agreement only for intact processes.
On the other hand,
the consensus protocol in this paper 
provides weak validity,
and
provides agreement for all well-behaved processes.
☞{We still have all these properties?}



% We note that 
% agreement for all well-behaved processes 
% versus only for intact processes
% our protocol validity, 
% does not provide validity:  all processes are well-behaved, the decision may not be a proposed value



% \textit{Federated (Byzantine) quorum systems (FBQS)
%     \cite{mazieres2015stellar,garcia2018federated}. \ }
% % 
% An FBQS lets 
% each process $p$ specify subjective sets of processes called slices.
% % 
% % A heterogeneous quorum system can be the result of sharing subjective slices
% % 
% % Each process $p$ specifies a set of slices.
% A slice is a subset of processes that
% % the process
% $p$ trusts when they state
% % a statement together.
% the same statement.
% A quorum is 
% % defined as 
% a set of processes that contains a slice for each of its members.
% %
% A process can construct a quorum starting from one of its own slices,
% % as the initial set, 
% and iteratively probing and including a slice of each process in the set.
% %
% % Each process in a heterogeneous quorum system needs to know only its own set of quorums.
% % ☞{The following is not true. Is that right?
%     % The resulting heterogeneous quorum system has quorum subsumption
%     % }
% % heterogeneous quorum system with 



% % \textbf{∗Classes of heterogeneous quorum systems. \ }
% \myparagraph{Classes of HQS}
% % 
% We now see a few related classes of quorum systems and 
% % the properties that they require.
% their properties.


% \textit{Dissemination quorum systems (DQS). \ }
% A DQS
% \cite{malkhi1998byzantine}
% declares a global set of quorums for all processes,
% and 
% % a set of Byzantine failure scenarios.
% a set of possible Byzantine sets.
% % global failure prone sets.
% % ☞{cite}
% % 
% A DQS is available for all well-behaved processes $𝓦$
% since it requires that
% there is at least one quorum that does not intersect 
% with any Byzantine set $𝓑$.
% It has quorum intersection
% % is consistent at $𝓦$
% since 
% it requires that
% the intersection of no pair of quorums falls completely in a Byzantine set $𝓑$.
% % 
% % It is weakly available for $𝓦$
% %It is available for $𝓦$
% %since there is at least one quorum that does not intersect 
% %with any Byzantine set.
% % 
% It is quorum subsuming for $𝓦$
% since the quorums are global:
% all the members of a quorum $q$ recognize $q$ as their own individual minimal quorum.
% % 
% % Therefore, it is available for $𝓦$.
% % 
% % Classic quorum systems are consistent, and available for all well-behaved processes
% % since every pair of $2f+1$ processes intersect,
% % and
% % there is at least one set of well-behaved processes of size $2f+1$.
% % 
% % Dissemination quorum systems are outlive for all the well-behaved processes.
% % 
% On the other hand,
% % heterogeneous quorum systems 
% HQSs
% may have
% % available and 
% quorum intersection, availability and inclusion only for a subset of well-behaved processes.
% % Therefore, they may be outlive only for a subset of them.
% % well-behaved processes.

%\xl{PBQS are HQS or not? It's domain does not exclude Byzantine processes.}




Personal Byzantine quorum systems (PBQS) \cite{losa2019stellar} 
capture the quorum systems that FBQSs derive form slices,
and
propose a consensus protocol.
% Further, 
% They left an open question about the weakest necessary condition for quorum systems to solve consensus that we answered in \autoref{sec:necess-prop}.
% 
They define a notion called quorum sharing
which requires quorum subsumption for every quorum.
% similar to quorum subsumption
On the other hand, 
in this paper, we show that even if a quorum system does not satisfy quorum sharing,
safety can be maintained for all processes,
and liveness can be maintained for the set of strongly available processes.
% however, (as we saw in \autoref{sec:prop-q-sys})
% quorum subsumption is weaker.
% as it requires inclusion only for well-behaved processes.
% Our protocols showed that quorum subsumption is sufficient to satisfy 
% reliable broadcast and consensus abstractions. 


% \textit{Personal Byzantine quorum systems (PBQS). \ }
% % 
% A PBQS
% % personal quorum system 
% \cite{losa2019stellar} is an HQS
% % quorum system
% that has quorum intersection, quorum availability, and quorum sharing within well-behaved subsets of processes which are called consensus clusters.
% % PBQS also has quorum availability inside consensus cluster.




When Byzantine processes don't lie about their slices,
an FBQS 
% The Federated Byzantine quorum system 
enjoys quorum sharing \cite{losa2019stellar}.
% (A similar observation is made about PBQSs \cite{losa2019stellar}.)
% ☞{This is proof for quorum sharing not quorum subsumption?}
% 
% By the protocol above,
Consider a quorum $q$ of a process $p$, and a process $p'$ in it.
Since 
a set is recognized as a quorum only if it contains a slice for each of its members,
the process 
$p'$ has a slice $s$ in $q$.
Processes receive the same set of slices from a given process even if it is Byzantine.
If $p'$ starts from $s$, 
it can find a quorum that grows no larger than $q$,
\ie, it can stop at $q$ if not earlier.
Therefore, $q$ includes a quorum of $p'$.
    

    
However, when Byzantine processes lie about their slices, FBQS does not satisfy quorum sharing.
Consider an FBQS with five processes 
$\P = \{1, 2, 3, 4, 5\}$,
and one Byzantine process $𝓑 = \{ 4 \}$.
% 
The slices of well-behaved processes $\W = \{1, 2, 3, 5\}$ are the following: $\S(1) = \{\{1, 2\}\}$, $\S(2) = \{\{2, 3\}, \{2, 4\}, \{2, 5\}\}$, $\S(3) = \{\{3, 4\}\}$, $\S(5) = \{\{2, 5\}\}$.
However, the Byzantine process $4$ provides different quorum slices to different well-behaved processes. 
The slices that it sends to each other process are the following: $\S(4)_1 = \{\{1, 4\}\}$, $\S(4)_2 = \{\{3, 4\}\}$, $\S(4)_3 = \{\{2, 4\}\}$, $\S(4)_5 = \{\{4, 5\}\}$.
By the definition of quorums in FBQS, 
% and the local view of each process
we have the following individual minimal quorums for each well-behaved process:
$\Q(1) = \{\{1, 2, 4\}, \{1, 2, 5\}\}$, $\Q(2) = \{\{2, 3, 4\}, \{2, 5\}\}$, $\Q(3) = \{\{2, 3, 4\}\}$, $\Q(5)$ $=$ $\{\{2, 5\}\}$.
We can see that $\Q$ does not have quorum sharing,
since the quorum $\{1, 2, 4\}$ does not include any quorum for process $2$.
However, $\Q$ is strongly available for processes $\{1, 2, 5\}$,
since they all have quorums that are well-behaved and quorum subsuming.
% 
Notice that abstract quorums which are over-approximations of FBQS satisfy quorum-sharing \cite{losa2019stellar}: A set $q$ is an abstract quorum of a process $p$ if $p$ is Byzantine, or $p$ has a slice contained in $q$ and every well-behaved member of $q$ has a slice contained in $q$.
However, as shown in our example, not all abstract quorums of a process can be observed by that process when Byzantine processes lie about their quorum slices.
For example, $\{1, 2, 4\}$ is an abstract quorum of process $2$ but $2$ does not observe it when the Byzantine process $4$ lies. 
Therefore, relaxation of the quorum sharing is necessary when analyzing 
quorum systems such as FBQS when Byzantine processes lie.
% 







Asymmetric Byzantine quorum systems (ABQS)
\cite{cachin2020asymmetric,cachin2020symmetric,alpos2021trust}
allow each process to define a subjective dissemination quorum system (DQS),
in a globally known system,
present shared memory and broadcast protocols,
and 
further, 
% presents 
rules to compose two ABQSs.
% where the global state of the two ABQSs is available.
%
On the other hand,
this paper 
lets each process specify its own set of quorums with only partial information about the system,
prove impossibility results, and presents protocols for reliable broadcast and consensus abstractions.
% and
% presents decentralized leader election algorithm.

We contrast HQS from ABQS on the following three aspects:
1) ABQS is based on asymmetric failure prone sets $Fᵢ$ from each process $pᵢ$. 
The notions of consistency and availability are dependents on the $Fᵢ$ sets . 
In contrast, HQS, and its consistency and availability properties are not dependent on failure prone sets. 
☞{HQS Special case of ABQS}
☞{B is what really happens not what people think, we can repeat analysis.}
% The byzantine scenarios B is the actual byzantine sets that can be tolerated.
2) The maximal strongly available set (from this work) is a strict superset of a maximal guild (from ABQS): 
☞{Is this too general to say?}
all the maximal guilds in ABQS are strongly available in HQS with quorum intersection; however, the opposite is not true.
We show a quorum system that has an empty guild but has non-empty strongly available set and quorum intersection.
Let $\P = \{1, 2, 3, 4\}$, and process $3$ is Byzantine. 
Let the asymmetric failure prone system be $\F(1) = \{\{3, 4\}, \{2\}\}$, $\F(2) = \{\{3, 4\}, \{1\}\}$, $\F(3) = \{\{1, 2\}\}$, $\F(4) = \{\{2, 3\}\}$. 
The canonical quorum systems are $\Q(1) = \{\{1, 2\}, \{1, 3, 4\}\}$, $\Q(2) = \{\{1, 2\}, \{2, 3, 4\}\}$, $\Q(3)= \{\{3, 4\}\}, \Q(4) = \{\{1, 4\}\}$. 
This HQS has quorum intersection and a non-empty strongly available set:
all the quorums of well-behaved processes have at least one correct process in their intersection. 
The set $\{1, 2\}$ is a strongly available set for $\Q$. 
However, it is not an ABQS with generalized $B^3$ condition. 
%However, the condition $B^3$ does not hold. 
For processes $1$ and $2$, $\F_1 = \{2\}, \F_2 = \{1\}$ and $\F_{12} = \{3,4\}$, and we have $\P ⊆ \{2\} \cup \{1\} \cup \{3, 4\}$, which violates generalized $B^3$.
Therefore this quorum system is not an ABQS. There is no guild set.
% 
3) HQS provides strictly stronger guarantees with weaker conditions. 
In ABQS, the consistency, validity, integrity, and totality properties are stated for wise processes (and guild), which are a subset of well-behaved processes with correct failure assumptions. 
For example, totality states that if a wise process delivers, then all processes in the maximum guild (that are all wise) deliver.
However, as stated in section 4 and 6.1, this paper states these four properties of the reliable broadcast for well-behaved processes.
For example, totality states that if a well-behaved process delivers, 
then well-behaved processes that are strongly available deliver. 
Well-behaved processes are a superset of wise processes. 
As noted above, strongly available set is a superset of guild.
Therefore, the BRB abstraction of this paper is stronger than ABQS's reliable broadcast.
	
%Regarding the asymmetric Byzantine reliable broadcast protocol, all the processes are linked by reliable and authenticated point-to-point FIFO channels. 
%In the Byzantine reliable broadcast protocol of this paper, no message is directly sent to all processes, it is only sent to the followers (line 14, 17, 20). 
%Further, in HQS, the axiom of locality states that a process only changes its local states when it receives messages from its quorum members, which does not require processes to be directly pair-wise connected.



Flexible BFT \cite{malkhi2019flexible} 
allows different failure thresholds between learners,
and
introduces 
% a new fault type called alive-but-corrupted and 
% a BFT 
a consensus protocol that
% that is resilient to these     faults 
guarantees safety only for learners with correct trust assumptions.
Heterogeneous Paxos (\cite{sheff2021heterogeneous}, \cite{sheff2014distributed}) further generalizes the separation between learners and acceptors with different trust assumptions;
it specifies quorums as sets rather than number of processes.
% 
It also proposes a consensus protocol that guarantees termination only for learners with correct trust assumptions.
Both of the two previous works are orthogonal to our paper
since they require the knowledge of all the processes in the system.
In contrast, HQS only requires partial knowledge of the system, 
and defines properties of quorum systems 
where reliable broadcast and consensus protocols are possible.
Multi-threshold reliable broadcast and consensus \cite{hirt2020multi}
and MT-BFT \cite{momose2021multi}
elaborate Bracha \cite{bracha1985asynchronous}
to have different fault thresholds for different properties and different synchrony assumptions.
% but 
However, they have cardinality-based or uniform quorums across processes.
HQS is more general since it supports 
% not-uniform 
heterogeneous sets of quorums.
% However, their quorums are still cardinality-based quorums.
% HQS is more general since quorums are represented by sets.



% protocol that can locally total orders proposals after a reliable broadcast.
% 
% when the sender is Byzantine 
% and the system members have heterogeneous trust.
% 
% We showed that 
% quorum subsumption is sufficient for 
% consistency and 
% availability of quorum systems, and 
% our reconfiguration protocols can preserve it.
K-consistent reliable broadcast (K-CRB) \cite{bezerra2022relaxed} introduces a relaxed reliable broadcast abstraction where the correct processes can define their own quorum systems without the complete knowledge of membership.
Given a quorum system, it focuses on
% K-CRB focuses on finding the strongest problem that can be solved in the HQS model:
% correct processes can deliver up to $k$ different values for an instance of K-CRB.
delivering the smallest number $k$ of different values.
% for an instance of K-CRB.
% 
In contrast, we propose the weakest condition 
to solve classical reliable broadcast and consensus in the HQS setting.
Moreover, K-CRB's relaxed liveness guarantee (accountability) requires public key infrastructure.
In contrast, all the proofs and protocols in this paper are designed for information-theoretic setting, where signatures are not available.
 



% ☞{Did we make the differences clear?}

% quorums are uniform across processes.
% do not allow heterogeneous quorums across processes.
% validity, totality and consistency respectively. 
% 
% seperate four fault thresholds for safety and liveness under synchrony and asynchrony to capture heterogeneity in the quorum systems.

% However, safety is only guaranteed between learners with correct trust assumption.


\begin{comment}
    Impossibility
    C0: Intact
    Strong Totality, if well-behaved delivers, then all the intact processes deliver.
    ——
    Weak weak Inclusion: only inside the intact.
    Intersection is strong, at Intact, We think that this is strong to provide strong totality.
    
    C1: cluster, instaniation
    Weak Totality, within consensus cluster
    ——
    Intersection is weaker, at a well-behaved.
    Strong inclusion: for all well-behaved. Subset required without intersection with well-behaved.        
    
    C2: weakset condition
    Weak Totality,
    ——
    Intesection, not considered here.
    Weak weak inclusion, only inside that set        
    ——
    Two first properties of intact: One well-behaved quorum with inclusion.
    that is the same as
    Weak availability and inclusion (Availability) for a set.
    
    Outlive
    Weak Totality, within O, similar to clusters
    ——
    Intersection is weaker, at a well-behaved.
    Weaker inclusion, for all well-behaved, interseciton with well-behaved                
    
    
    Inclusion: Intact < Ours (outlive) < Cluster
    
    Stronger
    C1               Solvable
    .                  ?
    .                  ?
    C1 and C0 are not comparable because of intersection.
    C0 Intact    Solvable
    C2               
    .                 Not solvable
    Weaker
    
    Open problem for the weakest condition.
    Is there any condition weaker than C1 such that consensus is solvable?    
    Ours
    With anything weaker than C2, consensus is not solvable. We have a theorem that shows a lower bound.
    Then we say that stellar is correct with this weak condition.
    This condition is both necessary and sufficient for availability of consensus.
    That shows that stellar protocol is the best than be done, closing the gap for availability of consensus.
    
    New problem: The Stellar paper states and provides stonger totality. Is intersection at intact needed for that?
    
    Abstract quorum system
    FBQS satisfies Abstract quorum system? No because of Byzantine lying about slices.
    With abstract quorum systems, you cannot get all of them. You need all for inclusion.
    The only thing that holds is the weakest condition similar to intact.
    
    They do not have the notion of abstract quorum subsumption. But if they did, their idea of caring only about W is similar to our intersection with W.
    
    Note: We may not need to compare outlive with intact or cluster.
    Intact is at a lower level for slices.
    Cluster is stronger because of inclusion and we already mentioned that.
    We said that outlive is simply the conjunction of the three properties.
    
\end{comment}


\begin{comment}
    
    Cobalt, Ripple
    UNL, Assume overlap more than 60\%, 90\%, assumed
    One trusted by everyone (Other paper mentioned)
    Limited decentralization
    Don't decentralized reconfiguration.
    
    Stellar
    Stellar system uses thresholds and hierarchies
    FBQS Stellar paper and 
    Model of FBQS paper
    both uses slices.
    Does not preserve Consistency, Fork has happened. Detected only after periodic check.
    Inclusion for intact if Byzantine do not lie about their slices, we mean inclusion out of intact is not guaranteed?
    
    Personal
    Works with quorums rather than slices
    They propose a consensus protocol.
    Assumes strong inclusion, inclusion of all members of quorums rather than the well-behaved processes. They require inclusion for Byzantine processes. Too strong. Even if they had recofig, they could not preserve inclusion.    
    We found the weakest condition for consensus
    
    Asymmetric
    Composition not reconfiguration interface
    Exchange of *global* quorum systems failure-prone set
    They do not have decentralized reconfiguration protocol. Need consensus? 
    They have protocol in text. (Maybe not correct: They do not have reconfiguration protocol (Decentralized protocol))
    
\end{comment}











% The Heterogeneous quorum systems are raised to attention for their usage in the permissioned blockchain.
% Ripple \cite{schwartz2014ripple} and Cobalt \cite{macbrough2018cobalt} are atomic broadcast protocols with non-uniform trust and no global membership information.
% Their safety relies on enough percentage of "overlap" between the unique node list or UNL, which is always guaranteed.
% However, the liveness is probabilistically guaranteed to be eventually 1 in the presence of maximal faults and asynchrony.
% % 
% Stellar \cite{mazieres2015stellar} is a Byzantine agreement protocol with no uniforms trust assumption among processes in the quorum system.
% However, there is no guarantee for consistency when reconfiguration happens excepts a "global intersection check".
% Both Ripple and Stellar relies on some threshold with hierarchy in practice (\cite{lokhava2019fast}) to maintain blockchain safety, which provides limited decentralization (\cite{bracciali2021decentralization} \cite{florian2022sum}). 
% Federated Byzantine quorum system \cite{garcia2018federated} generalizes and compares Stellar's federated voting and Bracha's Byzantine reliable broadcast (\cite{bracha1985asynchronous}).
% \cite{garcia2019deconstructing} analysis of the correctness of Stellar consensus.
% Personal Byzantine quorum system \cite{losa2019stellar} is an abstraction of Stellar Network and proposes a new consensus algorithm.
% However, they leave an open question about whether their construction of a consensus cluster is optimal for Byzantine consensus.
% We answer this question by proving the weakest condition for both consistency and liveness.
% Asymmetric Byzantine quorum systems (\cite{cachin2021asymmetric}, \cite{cachin2020symmetric}) share the non-uniformed trust insight as our heterogeneous quorum systems. 
% However, when reconfiguration $->$ composition happens, the personal fail-prone systems need to be exchanged and all the participants need to reach a consensus and adopt others' opinions(\cite{alpos2021trust}). 





% % However, quorum subsumption property holds within well-behaved processes' own views.
% We have both weak availability and quorum subsumption for intact set, which leads to full liveness for intact set.


\textbf{∗Impossibility Results.\ }
% 
There are two categories of assumptions about the computational power of Byzantine processes.
In the information-theoretic setting, Byzantine process have unlimited computational resources.
While in the computational setting, Byzantine processes can not break a polynomial-time bound \cite{garay2020sok}.
In this work, our impossibility results fall in the information-theoretic category.
Whether the same conditions are sufficient for reliable broadcast and consensus in the computational setting is an interesting open question.


FLP \cite{fischer1985impossibility} proved that consensus is not solvable in asynchronous networks even with one crash failure.
Later, \cite{fischer1986easy}, \cite{lamport1982byzantine} and \cite{borcherding1996levels} proved necessary and sufficient conditions for consensus and reliable broadcast to tolerate $f$ Byzantine failures in partially synchronous networks.
If the number of processes should be more than $3f$ and the connectivity of the communication graph should be at least $2f + 1$.
However, these results apply for cardinality-based quorums, which is a special instance of HQS.
We generalize the reliable broadcast and consensus abstractions 
for HQS which supports non-uniform quorums, 
and prove impossibility results for them.



\begin{comment}
    Group membership, overview
    a lot of works
    Fixed
    same view of membership
    or 
    global quorums.
    Lead to fixed protocol, often degenerates to just removing or adding a node.
    
    Passive
    The requester does not do anything
    Detector?
    Reiter, only group membership, no communication
    
    Active    
    Generality of our work, even more general than DQS, and cardinality that these works are based on.
    
    DBRB \cite{guerraoui2020dynamic}
    Broadcast
    Group membership and keep a quorum system with intersection.                
    Majority?, cardinality.
    X They have views too, not need numbers
    
    Dynamic Byzantine Quorum Systems (DBQS) \cite{alvisi2000dynamic} at DSN
    Read and write quorums of a quorum system, Is it register?
    Cardinality
    When more failure happens, increase f, increase the quorum size, vice versa
    
    Dyno \cite{duan2022foundations}
    Replication
    Group membership and consistent quorum system (intersection)
    Cardinality.
    X They have views.
    
    SmartMerge \cite{jehl2015smartmerge} 
    Mixed? Quorum policies (quorum configurations), cardinality, write all read one.
    
    All need global membership and quorums
    We have decentralized protocols to propagate the change.
    
\end{comment}





% All the previous works are dependent on either a consistent view of membership or a global quorum system information accessible at all processes.
% None of the information is available in the heterogeneous quorum systems even without reconfiguration requests.
% Further, group membership or dynamic group communication services require quorum systems to be uniform and public.
% So do the changes to them.
% The reconfiguration primitive is only concerned about quorums of a process itself.
% And the updates do not need to be observed by all the processes in the system.




% A reconfiguration primitive is often a secondary product of group membership primitive .
% All the processes in the system have the same view of membership and quorum configurations are global and public.
% Therefore, reconfiguration service can be accomplished by applying a pre-defined quorum configuration to the consistent group members.
% For example, in cardinality quorum systems, any set of $2/3 n +1$ processes is considered as a quorum in a system with $n$ processes (\cite{castro1999practical}).
% %Notice that we are not concerned with the global membership of the system, which differs our protocol from group membership protocols and view-synchronization protocols. 
% %☞{Group member is about knowing all processes, ours is about updating the quorum system.}
% 
% 
% There are two approaches for reconfiguration in dynamic membership systems. 
% The passive approach let all the existing processes in the system detect the failure or newly added processes(\cite{reiter1996secure}). 
% Since it is proven that accurate membership is as strong as consensus (\cite{chandra1996impossibility,chockler2001group}).
% %The reconfiguration happens when at least $f+1$ process detects the failure or existence of a new process, which relies on a failure detector available at each process. 
% All the processes can reach a consensus on the membership and adjust the quorum accordingly.
% % 
% The leaving or newly added process will be active after catching up on the membership history with existing processes. 
% The optimistic approach lets processes that request reconfigurations be responsible for the synchronization.
% % 
% DBRB \cite{guerraoui2020dynamic} make the leaving processes remain in the system until their messages are delivered. Sender has to sync before leaving as well.
% % 
% Dyno \cite{duan2022foundations} enforces consistent group membership and the leaving or new processes broadcast their intention to existing members of the system.
% % 
% % 
% SmartMerge \cite{jehl2015smartmerge} define a merge function to automatically switch between different quorum configurations.
% % 
% \cite{alvisi2000dynamic} adjust the quorum threshold based on dynamic failure information.
% % 
% All the previous works are dependent on either a consistent view of membership or a global quorum system information accessible at all processes.
% None of the information is available in the heterogeneous quorum systems even without reconfiguration requests.
% Further, group membership or dynamic group communication services require quorum systems to be uniform and public.
% So do the changes to them.
% The reconfiguration primitive is only concerned about quorums of a process itself.
% And the updates do not need to be observed by all the processes in the system.



%More specifically, the leaving process will be responsible for coordinating to avoid endangering quorum intersection. 
%And the joining process will specify its quorum system instead of accepting from existing ones.
%Most of the existing reconfiguration protocols are for cardinality quorum systems, where quorums are implicitly defined as any subset of $2f+1$ processes. 
%Or there exists a predefined merge function for quorum switch. 
%The predefined global quorums can be automatically adapted to different membership configurations. 

%However, none of them is general enough to capture the heterogeneous trust assumptions and open membership configurations in the real world. 
%Another disadvantage is that cardinality-based quorum systems rely on a failure detector or the assumption that $f < 1/3n$ even for unknown processes.
%By using the $2f+1$ quorums or "read one write all" quorums, the reconfiguration primitives degenerate to group membership primitives. The main difference between these two primitives is whether a process can decide the quorums simply based on the current system membership. Group membership protocols can decide the quorums thanks to the uniform assumptions on failure situations. While the assumption is not true for reconfiguration protocols.

%\textbf{∗reconfiguration in blockchain}

% ☞{Question: Why don't we just use consensus to do reconfiguration? Are our protocols more efficient? How?}
% is a blockchain that supports dynamic availablity by using two sets of commiting rules corresponding to quorum-based consensus and proof-of-work blockchain.
% 
% PBFT, eventual liveness
% blockchain: can fork,






% % \subsection{\textbf{Impossibilities and Trade-offs}}
% \textbf{∗Impossibilities and Trade-offs.\ }
% % 
% The famous FLP \cite{fischer1985impossibility} paper proves that consensus is impossible in the asynchrony system even with one crash failure.
% Later \cite{chandra1996weakest} proves that the weakest confition to have consensus is the eventual perfect failure detector available.
% Both of the paper assume global membership.

\textit{Unknown participants.\ }
% Similarly,
CUP and BCUP \cite{cavin2004consensus,alchieri2008byzantine}
consider consensus in an environment with unknown participants;
however, in contrast to HQS,
they assume properties about the topology of the network and its connectivity,
and consider only uniform quorums.


% CUP \cite{cavin2004consensus} is the first paper that proves the One Sink Reducibility participant detector is necessary and sufficient to solve consensus with unknown participants with only crash failures.
% BCUP \cite{alchieri2008byzantine} extends the result to accomendate Byzantine failures and proposed k-One Sink Reducibility participant detector.
% However, both of the paper assume uniform quorum systems and a public failure threshold, which is not available in HQS.


% % HotStuff \cite{yin2019hotstuff} is a BFT consensus that has linear communication complexity with a correct leader after GST.
% % 
% DAG{-}Rider \cite{keidar2021all} is an asynchronous Byzantine Atomic Broadcast protocol that can locally total orders proposals after a reliable broadcast.
% % 
% % \cite{bano2019sok} mentions hybrid consensus in the blockchain. 
% % This paper mentions the research gap is traditional BFT protocols cannot accommodate open node participation and high churn, especially in the dynamic committee configuration.
% % They also mention that maintaining liveness and security in a dynamic intra-committee configuration setting is an open and neglected research area in the design of single-committee blockchains.
% % 
% % RapidChain \cite{zamani2018rapidchain} is a blockchain protocol that provides scalability via full sharding.
% % It has a reconfiguration protocol to periodically change committee members with the help of random numbers and proof-of-work puzzles.
% SpeedingDumbo \cite{guo2022speeding} is a synchronize BFT protocol that dramatically reduces latency. 


% \cite{graf2021security} defines partial consistency for blockchains without consistent global views.
% 
% \cite{momose2022constant} propose BFT consensus with dynamic participation.
% 
% \cite{gelashvili2021brief} proposes an asynchronous view change protocol that utilizes random function for leader election.
% 
% \cite{graf2020accountability} analyze accountability property of blockchains, which is strictly weaker than consistency property.




==> LeaderElection.tex <==
\newpageprime
\subsection{\textbf{Leader Election}}
\label{sec:leader-election}

%☞{The proof variable in the protocol ... }

After the sink discovery protocol, $\ProtoSink$ is a fixed set of well-behaved processes.
They are strongly connected despite Byzantine failures in the system.
They can communicate with each other and collect the process identities with a vaild proof.
Then based on a pre-defined order across all processes (for instance, smallest process identity), 
exponential timeout back-off and 
a round-robin leader election approach to exclude the Byzantine processes,
eventually all the processes in $\ProtoSink$ elect the same well-behaved leader.
Finally, they propagate elected leader to their followers to finish the leader election process.

\begin{algorithm}
    \caption{Eventual Leader Election}
    \label{alg:leaderelection}
    \DontPrintSemicolon
    \SetKwBlock{When}{when received}{end}
    \SetKwBlock{Upon}{upon}{end}
    \Implements $\colon$ \ $\LeaderProto$\;
    %\ \ \ $\request : \Leave$ \;
    \ \ \ $\response : \Elect(p)$
    
    \textbf{Variables:}   \;
    \ \ \ $Q$ \Comment{The individual minimal quorums of $\self$} \;
    \ \ \ $\insink : \mathsf{Boolean}$ \;
    \ \ \ $\proofLE : \mathsf{Set}[\text{Exchange or Extend messages}]$\;    
    \ \ \ $F : 𝓟$ \;    
    \ \ \ $\sink : \mathsf{Set}[𝓟]$ \;
    
    \Upon ($\insink = \true$){  
        $\apl(p) \ \request \ \Propagate(\self, \proofLE)$ \mbox{ for each} $p ∈ F$ \label{algLE:sendproof}
    }

    \Upon ($\response$ \mbox{$\apl (p)$}, \mbox{$\Propagate(p', \proofLE')$} ){
        \If{$\proofLE'$ is valid}{
            $\sink \leftarrow \sink \cup \{p'\}$ \;
            $\apl(p'') \ \request \ \Propagate(p', \proofLE')$ \mbox{ for each} $p'' ∈ F$\label{algLE:passproof} \;
        }
    }
    
    \Upon (After GST){  
        \If{$\insink = \true$}{
            $\response \ \Elect(p)$ such that $p \in \sink$ and is choosen based on pre-defined order \label{algLE:election1} \;
            $\apl(p') \ \request \ \PropagateF(p, Q)$ \mbox{ for each} $p' ∈ F$ \label{algLE:passF}\;
        }
    }

    \Upon ($\response$ $\overline{\mbox{$\apl(p)$}}$, \mbox{$\PropagateF(p', Q')$} from each $p \in q$ s.t. $q \in Q' \wedge \textcolor{blue}{Validate(q)}$ \label{algLE:receiveQ}){  
        $\response \ \Elect(p')$ \label{algLE:election2}\;
    }
    
\end{algorithm}

Each well-behaved process keeps the following local variables for leader election:
$Q$ stores the individual minimal quorums for $\self$.
The following three variables are output of the sink discovery protocol:
$\insink$ is a boolean variable that indicates whether $\self$ is in the sink component of the quorum graph;
$\proofLE$ is a set of $\Exchange$ or $\Extend$ messages that serve as a proof when $\insink$ is $\true$;
$F$ is the follower set for $\self$;
$\sink$ is a set of processes that are verified to be in the sink component of quorum graph.
Notice that $\sink$ variables are updated gradually and we only ensure that they eventually converge to the same value for all the well-behaved processes.

\begin{lemma}[Eventual Agreement]
% Eventual leader election protocol has eventual agreement: There is a time after which 
% Eventually 
% no two well-behaved processes trust different processes.
Eventually well-behaved processes trust the same leader.
\end{lemma}

There are two cases where leader $p$ is elected by a well-behaved process. We prove agreement for both cases.
In the first case, leader is elected by a process in $\ProtoSink$ at \autoref{algLE:election1}.
Eventually all the processes in $\ProtoSink$ have the same $\sink$ variable by the epidemic $\Propagate$ messages they send to each other.
Then based on a pre-defined order across all processes, they will elect the same leader.

In the second case, leader is elected by a process out of $\ProtoSink$ at \autoref{algLE:election2}.
A well-behaved process only elects a leader if it receives $\PropagateF$ messages from a minimal quorum $q$ with at least one well-behaved member.
By quorum intersection, the elected leaders are the same for all the well-behaved processes.


\begin{lemma}[Eventual Accuracy]
%     There is a time after which 
    Every well-behaved process with weak availability
    eventually
    trusts some well-behaved process.
\end{lemma}

Each process keeps a local variable to store the processes in $\ProtoSink$ in $\sink$.
By the definition of strongly connected component and \autoref{lem:acc-1} and \autoref{lem:acc-2}, $\ProtoSink \subseteq \Sink$ and can reach all the well-behaved processes in $\Sink$.
$p \in \ProtoSink$ sends out their identity and a valid proof to all the processes in their quorums at \autoref{algLE:sendproof}.
Any process receives the $\Propagate$ message verify the correctness of the proof and update $\sink$ variable. 
They also propagate the process identity they received and the proof to their quorum members at \autoref{algLE:passproof}.
After the global stabalization time, all the well-behaved processes in $\Sink$ will have the same $\sink$ variable and elect the same leader based on the pre-defined order at \autoref{algLE:election1}.
By \autoref{lem:lemma2}, every the well-behaved process with weak availability is the follower of a well-behaved minimal quorum.
By \autoref{lem:exchange_complete}, they will eventually receive the propagation message send at \autoref{algLE:passF} from the well-behaved minimal quorum.
%at \autoref{algLE:receiveQ}.
Then they elect the leader at $\autoref{algLE:election2}$.



\begin{comment}
    \textbf{∗Preservation of quorum intersection. \ }
    
    By \autoref{lem:outlive-min-inter},
    at the beginning of execution,
    every outlive heterogeneous quorum system
    has
    outlive minimal quorum intersection.
    % 
    % \begin{lemma}
        % \label{lem:exec-leave-min-inter}
        % Every 
        % execution of
        % an outlive quorum system that 
        If the reconfiguration protocols of the system
        preserve outlive minimal quorum intersection
        % with the $\Leave$ protocol
        then
        the whole execution 
        enjoys
        outlive minimal quorum intersection.
        % \end{lemma}
    % 
    % And then for inductive steps
    % by \autoref{lem:leave-pres-inter}.
    % 
    % 
    % 
    % \begin{lemma}
        % \label{lem:exec-leave-inter}
        % 
        % By \autoref{lem:exec-leave-min-inter} and 
        Further, 
        by \autoref{lem:lemma0},
        and the fact that 
        having an intersection with the outlive set is a superset-closed property,
        we have that
        every execution
        % every 
        % execution of
        % an outlive quorum system 
        % with the $\Leave$ protocol
        enjoys
        outlive quorum intersection,
        % \end{lemma}
    % 
    % 
    that by \autoref{lem:q-inter-inter}
    immediately implies quorum intersection.
    
    % \begin{lemma}
        % \label{lem:exec-leave-inter-final}
        % Every 
        % execution of
        % an outlive quorum system with
        % the $\Leave$ protocol
        % enjoys
        % quorum intersection.
        % \end{lemma}
    % 
    % By \autoref{lem:exec-leave-inter}
    % and
    % \autoref{lem:q-inter-inter}.
    
    In the following sections,
    we prove that 
    each reconfiguration protocol
    preserve outlive minimal quorum intersection.
\end{comment}

% ☞{Merge with the original definitions.}


==> Protocols.tex <==
% \clearpage
\section{Protocols}


\subsection{Reliable broadcast protocol}
\label{sec:proto-reliable-broad}

We use a modified Bracha protocol to show that quorum intersection, availability and inclusion together are sufficient for Byzantine reliable broadcast.

Upon receiving the broadcast request (at \autoref{alg:rb-request}), 
the sender broadcasts the value $v$ to all the processes at \autoref{alg:rb-to-all}.
Upon receiving the message from sender(at \autoref{alg:rb-received}), correct processes echo this messsage among its followers at \autoref{alg:rb-echo-send}.
%quorum members.
When a correct process receives a quorum of consistent echo messages at \autoref{alg:rb-echo-rec-q}, it sends ready messages to all its followers at \autoref{alg:rb-ready-send}. 
%quorum members.
A correct process can also send ready message with a different value from its echo message.
It sends the ready message when it receives consistent ready messages from a blocking set(at \autoref{alg:rb-ready-rec-blocking}).
When a correct process receives a quorum of consistent ready messages at \autoref{alg:rb-ready-rec-q}, it delivers $v$ and finishes the reliable broadcast at \autoref{alg:rb-delivery-response}.

\begin{algorithm}
%     \small
    \caption{Byzantine reliable broadcast}
    \label{alg:brb}
    \DontPrintSemicolon
    \SetKwBlock{When}{when received}{end}
    \SetKwBlock{Upon}{upon}{end}
    \Implements $\colon$ \ $\mathsf{Reliable Broadcast}$ \;
    \ \ \ $\request : \mathit{Broadcast}(v)$ \;
    \ \ \ $\response : \mathit{Deliver}(v)$
    
    \textbf{Variables:}  \;
    \ \ \ $Q$: $\P$ \Comment{The individual minimal quorums of $\self$} \;
    \ \ \ $\F : 𝓟$ \Comment{The followers of $\self$} \;
    \ \ \ $\mathit{echoed}, \mathit{ready}, \mathit{delivery} : \mathsf{Boolean} ←\false$ \;
    
    \Uses $\colon$ \;
    \ \ \ $\apl : \F ↦ \mathsf{PointToPointLink}$ \;
    
    \Upon(\request \ \mbox{$\mathit{Broadcast}(v)$ from sender} \label{alg:rb-request}) {
        $\apl(p)$ \request \ \mbox{$\mathit{BCast}(v)$} for each $p ∈ \P$ \label{alg:rb-to-all} \; 
    }
    
    \Upon(\response \ $\apl$, $\mathit{BCast}$ \mbox{($v$)} $\wedge \mathit{echoed} = \false$ \label{alg:rb-received}){
        $\mathit{echoed} \leftarrow \true$ \;
        \textcolor{blue}{$\apl(p) \ \request \ \mathit{Echo}(v)$ for $p \in \F$ \;} \label{alg:rb-echo-send}
    }
            
    \Upon(\response \ $\apl$, $\mathit{Echo}$ \mbox{($v$)} from every $p \in q \wedge$ \textcolor{blue}{$q \in Q$} $\wedge \mathit{ready} = \false$ \label{alg:rb-echo-rec-q}){
        $\mathit{ready} \leftarrow \true$ \;
        \textcolor{blue}{$\apl(p) \ \request \ \mathit{Ready}(v)$ for $p \in \F$ \;} \label{alg:rb-ready-send}
    }

    \Upon(\response \ $\apl$, $\mathit{Ready}$ \mbox{($v$)} \textcolor{blue}{from every $p \in \mathit{Blocking}$ \mbox{($\self$)} }$\wedge \mathit{ready} = \false$ \label{alg:rb-ready-rec-blocking}){
        $\mathit{ready} \leftarrow \true$ \;
        \textcolor{blue}{$\apl(p) \ \request \ \mathit{Ready}(v)$ for $p \in \F$ \;} \label{alg:rb-ready-send2}
    }

    \Upon(\response \ $\apl$, $\mathit{Ready}$ \mbox{($v$)} from every $p \in q \wedge$ \textcolor{blue}{$q \in Q$} $\wedge \mathit{delivered} = \false$ \label{alg:rb-ready-rec-q}){
        $\mathit{delivered} \leftarrow \true$ \;
        $\response \ \mathit{Deliver}(v)$ \label{alg:rb-delivery-response}\;
    }


    \end{algorithm}

We prove that this algorithm provides Byzantine reliable broadcast when the quorum system satisfies our conditions.

    
    %\textbf{Consistency}
    \begin{lemma}
    	The BRB protocol guarantees consistency for well-behaved processes.
    \end{lemma}
    
    \begin{proof}
    	 A well-behaved process only delivers a message when it receives a quorum of consistency ready messages.
    	If $p_1$ delivers $m_1$ with $q_1$ and $p_2$ delivers $m_2$ with $q_2$, then the correct process in $q_1 \cap q_2$ only sends ready messages with one value then $m_1 = m_2$.
    	%Because our quorum system has at least a well-behaved process in the intersection of any pair of quourms.
    \end{proof}
   
    
    %\textbf{Validity}
    \begin{lemma}
    	If the quorum system $\Q$ is strongly available for $P$, then BRB protocol guarantees validity for $P$.
    \end{lemma}

	\begin{proof}
		When a correct sender broadcasts a message $m$, the correct process $p$ that is available has a quorum $q$ that only has well-behaved members.
		They all echo the same message $m$ to their followers, including process $p$.
		Then process $p$ has a quorum of consistent echo message for $m$.
		Since strong availability requires every process $p' \in q$ has a quorum $q' \subseteq q$.
		By the same reasoning, $p'$ receives a quorum ($q'$) of consistent echo message for $m$.
		Then all the processes in $q$ send out ready messages to their followers.
		Process $p$ now has a quorum of consistent ready message and it delivers $m$.
	\end{proof}
    
    
    %\textbf{Totality}
    \begin{lemma}
    	If the quorum system $\Q$ is available for $P$, then BRB protocol guarantees totality for $P$.
    \end{lemma}

	\xl{strictly weaker than FBQS}

	\begin{proof}
		A correct process delivers a  message $m$ when it receives a quorum $q$ of ready message for $m$.
		By the quorum intersection, $q$ intersects with all the quorums in the system at at least one well-behaved process.
		Then for any correct process $p'$, $q \cap \W$ is blocking: 
		$\forall p' \in \W, \forall q' \in \Q(p'), q \cap q' \cap \W \neq \emptyset$.
		Let's assume that $p_i$ is the well-behaved process in the correct intersection.
		Since $p_i \in q'$, $p'$ is $p_i$'s follower. 
		All the correct processes in $q$ send ready messages to their followers which includes $p'$.
		Then $p'$ receives a blocking set of ready messages and starts sending ready messages to its followers.
		For an available process $p''$, it has a quorum that all the memebrs are well-behaved.
		Then $p''$ will receive the ready message from the quorum and deliver $m$.
		
	\end{proof}
    
    %\textbf{No duplication}
    
    \begin{lemma}
    	The BRB protocol guarantees no duplication for all the well-behaved processes.
    \end{lemma}

	\begin{proof}
		  Since all the correct processes only sends out ready message for one $m$, every correct process can only collect at most one quorum of consistent ready message and deliver $m$ once.
	\end{proof}
    
   % \textbf{Integrity}
    
    \begin{lemma}
    	The BRB protocol guarantees integrity for all the well-behaved processes.
    \end{lemma}

	\begin{proof}
		 We prove that at least a quorum of echo messages was received for $m$ before the delivery.
		If a correct process delivers a message $m$, $m$ appears in a quorum $q_r$ of ready messages.
		By assumption, there is a non-empty set of available processes.
		Let process $p$ be available with its quorum $q$  and $q$ is well-behaved and quorum subsuming.
		Then by quorum intersection, $q \cap q_r \cap \W \neq \emptyset$.
		Let $p_i$ be a member of $q \cap q_r \cap \W$ which sents the ready message for $m$.
		$m$ can only be sent by a correct process in a ready message after a quorum of echo messages received for $m$ or a blocking set of ready messages received for $m$.
		If it's the first case, we complete the proof.
		If it's the second case, we prove that $p_i$ is not blocked by Byzantine processes and the first ready message sent by the process in $q$ is from a quorum of echo messages.
		Let the blocking set be $b$.
		By the quorum subsumption, $\exists q_i \in \Q(p_i), q_i \subseteq q \subseteq \W \wedge b \cap q_i \neq \emptyset$.
		Since $b$ always includes a process in $q$, by induction, the first process in $q$ which sends a ready message is triggered by receiving a quorum of echo messages.
		And we complete our proof.
		%Let $p_{i'} \in b \cap q_i$.
		%There is a correct process
		
		%Then the first ready message for $m$ is sent by receiving a quorum of echo messages for $m$.
		Every quorum of a well-behaved process includes well-behaved process.
		Then the echo message is sent by the correct processs after receiving it from the sender. 
		If the sender is correct, $m$ was previously broadcast by it.
	\end{proof}

\subsection{Consensus}
\label{sec:proto-consensus}

We can build a consensus with two rounds of Byzantine reliable broadcast. 
The structure is the same as abstract stellar consensus protocol.
Each proposed value is associated with a round number in a ballot ($\langle r, v \rangle$).
Ballots are totally ordered by their round number and value.
For each process, we define four local variables: 
$\r$ is a integer which represents current round number.
$\candidate$ is a ballot that the process tries to commit.
$\prepared$ is a ballot that the process is safe to disgard any lower ballots.
$\ballots$ is a set of ballots that the process has seen so far.

%We use $\langle r, v \rangle$ to represent a ballot where $r$ is the round number and $v$ is a consensus value.
%We assume that $\langle r, v \rangle$ are totally ordered.
Then for the consensus protocol, in the first round of BRB, it aborts everything that is lower and incompatible with its current proposal $\candidate$ by vote $\false$ to those ballots.

For the second round of BRB, it tries to commit its own proposal.
If it receives $\false$ delivered for all the ballots $b'$ that are lower and incompatible with $b$ and $\prepared$ is lower than $b$, then $b$ is assigned to $\prepared$. 
We assign $\candidate$ in the same way.
Then the process can vote $\true$ for $\candidate$.

When a ballot is delivered to be $\true$, the process decide this value for consensus.

To provide liveness, a process will trigger a timeout for each round if no value is decided after a long time.
The process will increment the round number by one and use BRB to prepare the value in $\prepared$.
The timer is reset at the begining of each round, when a process received either a quorum of message to prepare a value or commit a value. 

\textbf{Agreement}

Agreement is guranteed by the consistency of BRB. 
A correct process only decides $b.v$ after the deliver of $\true$ for ballot $b$.
By the consistency of BRB, other correct process can only deliver $\true$ for the ballot $b$ and deliver the same value $b.x$.

\textbf{Weak validity}

If all the processes are correct and propose the same value $v$, then the consensus will end in the first round.
All the processes vote $\false$ for round $0$. 
By the validity of BRB, all the processes vote the same value is equivalent to a correct sender broadcast that value.
Then all the processes deliver $\false$ to ballot $\langle 0, \bot \rangle$ and prepare ballot $\langle 1, v \rangle$.
They vote $\true$ for ballot $\langle 1, v \rangle$ and by validity of BRB, all the processes deliver $\true$ for the same ballot and decide $v$.

If all processes are correct and some process decides a value $v$, then before the decision from consensus, $v$ was delivered in a ballot by the process.
Let assume the ballot is $\langle r, v \rangle$.
By the integrity of BRB, a correct process vote $\true$ for the ballot $\langle r, v \rangle$.
A correct process only vote $\true$ for its $\candidate$.
The $\candidate$ is asisgned with two potantial value: its own proposal or the $\prepared$ value.
If it's the first case, we proved the decision for consensus was proposed by a correct process.
If it's the second case, the $\prepared$ value is updated when a process BRB deliver $\false$ to all the ballots lower than $\prepared$.
By the integrity of BRB, some process vote $\false$ for the ballots lower than $\langle r, v \rangle$. 
Correct processes vote $\false$ only when they propose a value for consensus or trigger a time out for a round.
In the first case, we proved that $v$ was proposed by some process.
In the second case, the time out is set when a process receives a quorum of messages vote for a round $r' > r$.
By induction, the vote was from some process's proposal.


\xl{We may need to prove a variant of the integrity of BRB: if all the processes are correct and some process deliver a value, the that value was proposed by some process. The proof is the same as BRB's normal integrity, we only need to change the last step that the echo was sent by some correct process.}

\textbf{Weak liveness}

Eventually in a round all the correct processes propose the same value.
By the validity, totality and consistency of BRB, all the correct processes prepared the value and decide that value. 


==> ProtocolsEric.tex <==
% \clearpage
\section{Protocols}

We just showed that quorum intersection and quorum availability are not sufficient to implement our desired distributed abstractions.
Now, we show that our newly introduced property, quorum subsumption, along with quorum intersection and quorum availability are sufficient to implement both Byzantine reliable broadcast and consensus.
 

% Maybe you want to do something like: 
% Before we actually give the protocol, we recall an earlier example, that did not have quorum subsumption, and thus did not satisfy our specifications. 
% Now, we show that if quorum subsumption holds for that example, we do get our specifications... (migrate any of the blocks about quorum subsumption here)
% This is just to provide some intuition or to give a solid example, if possible.

\subsection{Reliable broadcast protocol}
\label{sec:proto-reliable-broad}
In \autoref{alg:brb},
we adapt the Bracha protocol \cite{bracha1985asynchronous} to show that quorum intersection, availability and inclusion together are sufficient for Byzantine reliable broadcast. The changed parts are highlighted in blue.

Each process stores the set of its individual minimal quorums $Q$,
and its set of followers $𝓕$.
It also stores the boolean flags 
$\mathit{echoed}$, $\mathit{ready}$, and $\mathit{delivered}$.
It further uses point-to-point links $\apl$ to each of its followers.
% 
Upon receiving a request to broadcast a value $v$ (at \autoref{alg:rb-request}), 
the sender broadcasts the value $v$ to all the processes (at \autoref{alg:rb-to-all}).
Upon receiving the message from the sender (at \autoref{alg:rb-received}), 
a well-behaved process echoes the message among its followers (at \autoref{alg:rb-echo-send}).
% \ec{should we define followers first?}
%quorum members.
When a well-behaved process receives a quorum of consistent echo messages (at \autoref{alg:rb-echo-rec-q}), it sends ready messages to all its followers (at \autoref{alg:rb-ready-send}). 
%quorum members.
A well-behaved process can also send a ready message 
% with a different value from its echo message.
% It sends the ready message 
when it receives consistent ready messages from a blocking set (at \autoref{alg:rb-ready-rec-blocking}).
When a well-behaved process receives a quorum of consistent ready messages (at \autoref{alg:rb-ready-rec-q}), it delivers $v$ 
% and finishes the reliable broadcast 
(at \autoref{alg:rb-delivery-response}).


\begin{algorithm}
%     \small
    \caption{Byzantine Reliable Broadcast (BRB)}
    \label{alg:brb}
    \DontPrintSemicolon
    \SetKwBlock{When}{when received}{end}
    \SetKwBlock{Upon}{upon}{end}
    \Implements $\colon$ \ $\mathsf{Reliable Broadcast}$ \;
    \ \ \ $\request : \mathit{Broadcast}(v)$ \;
    \ \ \ $\response : \mathit{Deliver}(v)$
    
    \textbf{Variables:}  \;
    \ \ \ $Q : 2^\P$ \Comment{The individual minimal quorums of $\self$} \;
    \ \ \ $\F : 𝓟$ \Comment{The followers of $\self$} \;
    \ \ \ $\mathit{echoed}, \mathit{ready}, \mathit{delivered} : \mathsf{Boolean} ←\false$ \;
    
    \Uses $\colon$ \;
    \ \ \ $\apl : \F ↦ \mathsf{PointToPointLink}$ \;
    
    \Upon(\request \ \mbox{$\mathit{Broadcast}(v)$ from sender} \label{alg:rb-request}) {
        $\apl(p)$ \request \ \mbox{$\mathit{BCast}(v)$} for each $p ∈ \P$ \label{alg:rb-to-all} \; 
    }
    
    \Upon(\response \ $\apl\mbox{($p$)}$, $\mathit{BCast} \mbox{($v$)} \wedge \mathit{echoed} = \false$ \label{alg:rb-received}){
        $\mathit{echoed} \leftarrow \true$ \;
        \textcolor{blue}{$\apl(p) \ \request \ \mathit{Echo}(v)$ for $p \in \F$ \;} \label{alg:rb-echo-send}
    }
            
    \Upon(\response \ $\apl\mbox{($p$)}$, $\mathit{Echo} \, \mbox{($v$)}$ from every $p \in q \; \wedge$ \textcolor{blue}{$q \in Q$} $\wedge \; \mathit{ready} = \false$ \label{alg:rb-echo-rec-q}){
        $\mathit{ready} \leftarrow \true$ \;
        \textcolor{blue}{$\apl(p) \ \request \ \mathit{Ready}(v)$ for $p \in \F$ \;} \label{alg:rb-ready-send}
    }

    \Upon(\response \ $\apl\mbox{($p$)}$, $\mathit{Ready} \, \mbox{($v$)}$ \textcolor{blue}{from every $p \in P$, $P$ is a blocking set of $\self$} $\wedge \; \mathit{ready} = \false$ \label{alg:rb-ready-rec-blocking}){
        $\mathit{ready} \leftarrow \true$ \;
        \textcolor{blue}{$\apl(p) \ \request \ \mathit{Ready}(v)$ for $p \in \F$ \;} \label{alg:rb-ready-send2}
    }

    \Upon(\response \ $\apl$, $\mathit{Ready} \, \mbox{($v$)}$ from every $p \in q \; \wedge$ \textcolor{blue}{$q \in Q$} $\wedge \; \mathit{delivered} = \false$ \label{alg:rb-ready-rec-q}){
        $\mathit{delivered} \leftarrow \true$ \;
        $\response \ \mathit{Deliver}(v)$ \label{alg:rb-delivery-response}\;
    }

\end{algorithm}

We prove that this protocol implements Byzantine reliable broadcast when the quorum system satisfies 
% the three conditions:
quorum intersection, and strong availability.
We remember that 
strong availability requires both weak availability and quorum subsumption.
More precisely, it requires
weak availability, \ie, 
a well-behaved quorum $q$ for a process $p$,
and 
quorum subsumption for $q$.

% for a non-empty set 
% availability and inclusion.
% \ml{inclusion for which quorum(s)?}


%\textbf{Consistency}
\begin{lemma}
    The BRB protocol guarantees consistency for well-behaved processes.
\end{lemma}

\begin{proof}
        A well-behaved process only delivers a message when it receives a quorum of consistency ready messages.
    If $p_1$ delivers $m_1$ with $q_1$ and $p_2$ delivers $m_2$ with $q_2$, then a well-behaved process in $q_1 \cap q_2$ only sends ready messages with one value. Thus, $m_1 = m_2$.
    %Because our quorum system has at least a well-behaved process in the intersection of any pair of quourms.
\end{proof}
   
    
%\textbf{Validity}
\begin{lemma}
    If the quorum system $\Q$ is strongly available for $P$, then BRB protocol guarantees validity for $P$.
\end{lemma}

\begin{proof}
    Consider a well-behaved sender that broadcasts a message $m$.
    By availability,
    the well-behaved process $p$
%     that is available 
    has a quorum $q$ that contains only well-behaved members.
%     
    They all echo the same message $m$ to their followers, including process $p$.
    Thus, process $p$ receives a quorum $q$ of consistent echo messages for $m$.
    By strong availability, 
    every process $p' \in q$ has a quorum $q' \subseteq q$.
%     
    By the same reasoning, 
    every process $p'$ receives a quorum $q'$ of consistent echo messages for $m$.
%     
    Thus, all the processes in $q$ send out ready messages to their followers.
%     
    Therefore, process $p$ receives a quorum of consistent ready message 
    and delivers $m$.
\end{proof}

% \xl{strictly weaker than FBQS}
% \ml{You want to add something here?}
    
%\textbf{Totality}
\begin{lemma}
    If the quorum system $\Q$ is available for $P$, then BRB protocol guarantees totality for $P$.
\end{lemma}

\begin{proof}
    We assume that a well-behaved process $p$ has delivered $m$, and show that every well-behaved process $p'$ delivers $m$.
    We show that every well-behaved process $p''$ sends ready messages to its followers.
    The well-behaved process $p$ delivers $m$ only when it receives a quorum $q$ of ready messages for $m$.
    By quorum intersection, $q$ intersects all quorums in the system in at least one well-behaved process.    
    Therefore, 
%     for any well-behaved process $p'$, 
    $q \cap \W$ is $p''$-blocking.
%     $\forall p' \in \W, \forall q' \in \Q(p'), q \cap q' \cap \W \neq \emptyset$.
    Consider a quorum $q''$ of $p''$.
    Let's assume that $p_i$ is the well-behaved process in the intersection of $q$ and $q''$
    Since $p_i$ is in $q''$, then $p''$ is a follower of $p_i$.
    All the well-behaved processes in $q$ send ready messages to their followers which includes $p'$.
    Thus, $p'$ receives a blocking set of ready messages,
    and starts sending ready messages to its followers.
    The well-behaved process $p'$ has a quorum with all well-behaved members.
    Thus, $p'$ will receive ready message from a quorum, and delivers $m$.
\end{proof}

% \ec{
% im missing the reasoning here, how does $p'$ sending ready to its followers 
% imply that every member in $q''$ of $p''$ receives ready?
% }

%\textbf{No duplication}

\begin{lemma}
    The BRB protocol guarantees no duplication for all the well-behaved processes.
\end{lemma}

\begin{proof}
    A well-behaved process keeps the $\mathit{delivered}$ boolean,
    and delivers a message at most once.
%     A well-behaved process delivers a message $m$ only when it receives a quorum of ready messages for $m$. By quorum intersection, every pair of quorums intersect at a well-behaved process. A well-behaved process keeps the $\mathit{ready}$ boolean and only sends out ready messages for one $m$. Therefore, a well-behaved process cannot deliver 
\end{proof}

% \textbf{Integrity}

\begin{lemma}
    The BRB protocol guarantees integrity for all the well-behaved processes.
\end{lemma}

\begin{proof}
    We assume that a well-behaved process $p$ delivers a message $m$ with a well-behaved sender process $p'$,
    and prove that (1) the process $p'$ has broadcast $m$.
     
    We first prove that 
    (2) a well-behaved process $p_e$ has received of echo messages
    from at least a quorum $q_e$ of $p_e$.
%     
    Since the well-behaved process $p$ delivered $m$, 
    it has received a quorum $q_r$ of ready messages.
    By the strong availability assumption, 
    there exists a process 
%     $p$ 
    with a quorum $q$ that is well-behaved and quorum subsuming.
%     
    Then, by quorum intersection, 
%     $q \cap q_r \cap \W \neq \emptyset$.
    $q_r$ and $q$ intersect at a well-behaved process $p_i$.
%     Let $p_i$ be a member of $q \cap q_r \cap \W$ which sent the ready message.
    The process $p_i$ sent a ready message (that $p$ received).
    A well-behaved process $p_i$ sends a ready message only if it
    either receives echo messages from a quorum of $p_i$, 
    or receives ready messages from a $p_i$-blocking set $P$.
%
    If it's the first case, we proved (2) above.
    Let us consider the second case.
    By the quorum subsumption, since $p_i$ is in $q$, $p_i$ has a quorum $q_i$ that is a subset of $q$.
    Since $P$ is a blocking set of $p_i$,
    $P$ intersects with $q_i$.
    Therefore $P$ intersects with $q$.
%     $\exists q_i \in \Q(p_i), q_i \subseteq q \subseteq \W \wedge b \cap q_i \neq \emptyset$.  

    Let $p_f$ be the first process in $q$ that sent a ready message.
    A well-behaved process $p_f$ sends a ready message only if it
    either receives echo messages from a quorum of $p_f$, 
    or receives ready messages from a $p_f$-blocking set $P'$.
    If it's the first case, we proved (2) above.
    Let us consider the second case.
    With the same reasoning as for $p_i$,
    $P'$ intersects with $q$.
    Thus, $p_f$ has received a ready message from a process in $q$.
    Therefore, $p_f$ is not the first process in $q$ to send a ready message.
    This is a contradiction with the definition of $p_f$ above.

    We now use (2) above to prove (1) above: 
    the process $p'$ has broadcast $m$.
    %Then the first ready message is sent by receiving a quorum of echo messages.
    Since every quorum of a well-behaved process includes itself,    
    $q_e$ includes $p_e$.
%     
    Therefore, $p_e$ has received an echo message from itself.
    A well-behaved process sends an echo message only after receiving it from the sender $p'$. 
%     
    Since the sender $p'$ is well-behaved, 
    and $p_e$ has received the message $m$ from it,
    by the integrity of point-to-point links,
    $p'$ has previously sent $m$ to every process.
\end{proof}


\subsection{Consensus}
\label{sec:proto-consensus}

\begin{algorithm}
	%     \small
	\caption{Weak Byzantine Consensus (BC)}
	\label{alg:bc}
	\DontPrintSemicolon
	\SetKwBlock{When}{when received}{end}
	\SetKwBlock{Upon}{upon}{end}
	\Implements $\colon$ \ $\mathsf{Consensus}$ \;
	\ \ \ $\request : \mathit{propose}(v)$ \;
	\ \ \ $\response : \mathit{decice}(v)$
	
	\textbf{Variables:}  \;
	\ \ \ $Q$: $2^\P$ \Comment{The individual minimal quorums of $\self$} \;
	\ \ \ $\F : 𝓟$ \Comment{The followers of $\self$} \;
	\ \ \ $\mathit{round}: \mathbb{N}^{+} \leftarrow 0$ \Comment{Current round number} \;
	%\ \ \ $\mathit{echoed}, \mathit{ready}, \mathit{delivered} : \mathsf{Boolean} ←\false$ \;
	\ \ \ $\mathit{candidate}, \mathit{prepared} : \langle \mathbb{N}^{+}, V \rangle ←\langle 0, \bot \rangle$ \;
	\ \ \ $\mathit{leader} : 𝓟$ \Comment{current leader} \;
	%\ \ \ $\mathit{ProposeSet} : V$ \Comment{the set conatins proposed values} \;
	
	\Uses $\colon$ \;
	\ \ \ $\apl : \F ↦ \mathsf{PointToPointLink}$ \;
	\ \ \ $\brb : \P ↦ \mathsf{ByzantineReliableBroadcast}$ \;
	\ \ \ $\le : \P ↦ \mathsf{EventualLeaderElection}$ \;
	
	%\wedge \self = \mathit{leader}
	\Upon(\request \ \mbox{$\mathit{propose}(v)$} \label{algC:propose}) {
		%$\brb$ \ \request \ \mbox{$\mathit{Initial}(v)$} \; 
		$\mathit{candidate} \leftarrow \langle 1, v \rangle$ \label{algC:assign-proposal}\;
		\If{$\self = \mathit{leader}$}{
			$\for_all \ b' \not \preceq \mathit{candidate},$ 
			$\brb(b')$ \request \ \mbox{$\mathbb{A}$}  \label{algC:leader-abort}\; 
		}
	}

	%\Upon(\response \ $\mathit{Initial}$\mbox{$(v)$}){
		%$\mathit{ProposedSet} \leftarrow \mathit{ProposedSet} \cup v$ \;
	%}
	
	\Upon(\response \ $\brb$\mbox{$(b')$}, $\mathbb{A}$ from $\mathit{leader}$ for all $ b' \not \preceq b \wedge \mathit{prepared} \prec b$ \label{algC:prepared}){
		$\mathit{prepared} \leftarrow b$ \label{algC:update-prepared}\;
		%\If{$\mathit{candidate} \prec \mathit{prepared}$}{
			%$\mathit{candidate} \leftarrow \langle \mathit{round}, v'\rangle$, $v'$ is the smallest value $\geq \prepared.v$  \;
			\If{$\self = \mathit{leader}$}{
				\If{$\prepared = \candidate $ \label{algC:prepare-candidate}}{
				$\brb(\mathit{candidate}) \ \request \ \mathbb{C}$ \label{algC:leader-commit} \;
				}
				%\Else{
					%$\for_all \ b' \not \preceq \mathit{candidate}, \brb(b')$ \request \ \mbox{$\mathbb{A}$ \label{algC:leader-continu-abort}} \; }
			%}
		}
	}

	\Upon(\response \ $\brb$\mbox{$(b)$}, $\mathbb{C}$ from $\mathit{leader} \wedge b = \prepared$ \label{algC:commit-prepared}){
		$\response \ \mathit{decice}(b.v)$ \label{algC:decision-reponse}\;
	}


	\Upon($\mathit{timeout}$ triggered \label{algC:trigger-timer}){
		$\le \ \request \ \mathit{Complain}(\mathit{round})$\;
	}

	\Upon($\le \ \response \ \mathit{NewLeader}$ \mbox{($p$)}\label{algC:new-leader}){
		$\mathit{leader} = p$ \;
		$\mathit{round} \leftarrow \mathit{round} + 1$ \label{algC:increase-round}\;
		start-timer($\mathit{round}$) \label{algC:reset-timer} \;
		%\If{$\mathit{prepared} = \langle 0, \bot \rangle$}{
			$\mathit{candidate} \leftarrow \langle \mathit{round}, \mathit{candidate}.v\rangle$ \label{algC:update-candidate}\;
		%}
		%\Else{ 			
			%$\mathit{candidate} \leftarrow \langle \mathit{round}, \candidate.v\rangle$  \;
			%$\mathit{candidate} \leftarrow \langle \mathit{round}, v'\rangle$, $v'$ is the smallest value $\geq \prepared.v$  \;
			%$\mathit{candidate} \leftarrow \langle \mathit{round}, \mathit{prepared}.v\rangle$ \;
		%}
	\If{$\self = p$ \label{algC:self-new-leader}}{
		$\for_all \ b' \not \preceq \mathit{candidate}$, 
		$\brb(b')$ \request \ \mbox{$\mathbb{A}$} \label{algC:abort-new-round}\; 
	}
	}



\begin{comment}
		\Upon($\exists q \in Q \wedge \self$ received messages for round $r' > r$ from $\forall p \in q$ ){
		$\mathit{round \leftarrow \text{min}\{r' | r' = b'.r \wedge b' \text{received from} \ q}\}$ \;
		start-timer($\mathit{round}$) \;
	}
	
	\Upon($\mathit{timeout}$ triggered){
		\If{$\mathit{prepared} = \langle 0, \bot \rangle$}{
			$\mathit{candidate} \leftarrow \langle \mathit{round + 1}, \mathit{candidate}.v\rangle$ \;
		}
		\Else{ 			
			$\mathit{candidate} \leftarrow \langle \mathit{round + 1}, \mathit{prepared}.v\rangle$ \;
		}
		$\for_all \ b' \not \preceq \mathit{candidate}$, 
		$\brb(b')$ \request \ \mbox{$\mathbb{A}$} \; 
	}

	\Upon($\mathit{timeout}$ triggered){
	\If{$\mathit{prepared} = \langle 0, \bot \rangle$}{
		$\mathit{candidate} \leftarrow \langle \mathit{round + 1}, \mathit{candidate}.v\rangle$ \;
	}
	\Else{ 			
		$\mathit{candidate} \leftarrow \langle \mathit{round}, v'\rangle$, $v'$ is the smallest value $\geq \prepared.v$  \;
		%$\mathit{candidate} \leftarrow \langle \mathit{round + 1}, \mathit{prepared}.v\rangle$ \;
	}
	$\for_all \ b' \not \preceq \mathit{candidate}$, 
	$\brb(b')$ \request \ \mbox{$\mathbb{A}$} \; 
}
\end{comment}

\end{algorithm}

We can build a consensus with two rounds of the Byzantine reliable broadcast
that we saw in the previously subsection. 
The structure is samilar to the abstract stellar consensus protocol \ml{\cite{garcia2019deconstructing}}.
We present an overview of the protocol, and 
prove that, in an HQS with quorum intersection and strong availability,
it satisfies the consensus specification.

\ec{
We can build a consensus protocol using the Byzantine reliable broadcast abstraction we just saw.
Each process enters the consensus protocol with a proposed value $v$.
We assume the existence of an eventual leader election protocol that will eventually elect a well-behaved process as the leader, an infinite amount of times.
We first preseent an overview of the protocol, then prove that in an HQS with quorum intersection and strong availability, it satisfies the consensus specifications.
}


Each proposed value $v$ is associated with a round number $r$ in a ballot $\langle r, v \rangle$.
Ballots are totally ordered by their round number and value.
Each process stores the following four local variables: 
$\r$ is an integer representing the current round number,
$\candidate$ is a ballot that the process tries to commit,
$\prepared$ is a ballot that the process is safe to discard any ballots lower than it,
and
$\mathit{leader}$ is the output from the eventual leader election module.
%\ec{was there another variable you forgot to include?}
%$\ballots$ is a set of ballots that the process has seen so far.

\ec{
When a process $p$ is the designated leader, it will try to get its value $v$ decided.
}


%We use $\langle r, v \rangle$ to represent a ballot where $r$ is the round number and $v$ is a consensus value.
%We assume that $\langle r, v \rangle$ are totally ordered.
Upon receiving a propose request at \autoref{algC:propose},
a well-behaved process assign its proposal to the a candidate ballot at \autoref{algC:assign-proposal}.
If $\self$ is the leader, it prepares its $\candidate$ by broadcasting $\mathbb{A}$ messges for all the ballots that are below $\candidate$ at \autoref{algC:leader-abort}.
When a well-behaved process delivers $\mathbb{A}$ messages for all the ballots below $b$ from the leader and it has not prepared $b$(at \autoref{algC:prepared}), 
it updates its $\prepared$ variable to the ballot $b$ at \autoref{algC:update-prepared}.
If $\self$ is the leader and the $\prepared$ variable is equal to $\candidate$ variable, 
$\self$ boradcasts $\mathbb{C}$ message for its $\candidate$(at \autoref{algC:leader-commit}).
If not, $\self$ waits for $\prepared$ variable to be updates by other $\mathbb{A}$ messages.


When a well-behaved process delivers $\mathbb{C}$ message for a ballot $b$ and it already prepared the same ballot(at \autoref{algC:commit-prepared}), 
it decides the value of that ballot and issues response (at \autoref{algC:decision-reponse}).


To provide liveness, well-behaved processes will trigger timeout for each round if no value is decided after a long time and complain to the leader election module (at \autoref{algC:trigger-timer}).
When the leader election module output a new leader(at \autoref{algC:new-leader})
a well-behaved process increment the round number by one and update the $\mathit{leader}$ variable at \autoref{algC:increase-round}.
It also reset the timer and double the time-out period at \autoref{algC:reset-timer}.
The $\candidate$ varible is updated with the new round number at \autoref{algC:update-candidate}.
If $\self$ is the new leader, it broadcast $\mathbb{A}$ messages for all the ballots below than its $\candidate$ at \autoref{algC:abort-new-round}.



%\textbf{Agreement}
\begin{lemma}[Agreement]
	The consensus protocol guarantees agreement for well-behaved processes.
\end{lemma}

\xl{stronger than abstarct consensus}

\begin{proof}
	We prove agreement by contradiction.
	Assume that there are two well-behaved processes deliver two different values.
	Let process $p$ deliver $v$ in ballot $b$ and let process $p'$ deliver $v'$ in ballot $b'$.
	Since ballots are totally ordered, without generality, we asusme that $b \not \preceq b'$.
	Process $p'$ can only deliver $v'$ at \autoref{algC:commit-prepared} and it checks $b'$ has been prepared.
	A well-behaved process prepare a new ballot $b'$ after aborting all the ballots below and incompatible with $b'$ at \autoref{algC:prepared}.
	Since $b \not \preceq b'$, $p'$ delivers the $\mathbb{A}$ message for $b$ before $b'$ is prepared.
	However, since process $p$ decides $v$ with $b$ at \autoref{algC:commit-prepared}, $p$ delivers $\mathbb{C}$ mesage for $b$.
	For the same BRB instance with ballot $b$, two well-behaved processes deliver conflict values $\mathbb{A}$ and $\mathbb{C}$, which violates the consistency property of BRB.
	We reach a contradiction and proved that two well-behaved processes can not decide different values. 
	
	%Agreement is guranteed by the consistency of BRB. 
	%A well-behaved process only decides $b.v$ after the deliver of $\mathbb{C}$ for ballot $b$ and $b$ is the prepared ballot.
	%By the consistency of BRB, other well-behaved process can only deliver $\mathbb{C}$ for the ballot $b$ and deliver the same value $b.x$.
\end{proof}


%\textbf{Weak validity}
\begin{lemma}[Weak validity]
	The consensus protocol guarantees weak validity for well-behaved processes.
\end{lemma}

\xl{stronger than the abstract consensus}

\begin{proof}
	
	When a well-behaved process decides a value $v$ at \autoref{algC:decision-reponse}, $v$ was delivered in a $\mathbb{C}$ message for a ballot $b$ and $b.v = v$(at \autoref{algC:commit-prepared}).
	Since all the processes are well-behaved including the leader, by integrity property of BRB,
	the leader broadcasts $\mathbb{C}$ message for the ballot $b$ at \autoref{algC:leader-commit}.
	Ballot $b$ is leader's $\candidate$ by the condition at \autoref{algC:prepare-candidate}.
	The value for the $\candidate$ ballot is assigned with its initial proposal at \autoref{algC:assign-proposal} and it never changes this value.
	Thus $v$ was proposed by the leader at \autoref{algC:propose}.
	If all the processes are well-behaved and propose the same value inclduing the leader, then $v$ is the proposed value.
	If all the processes are well-behaved, then $v$ was proposed by some well-behaved process, which is the leader.
	%If all the processes are well-behaved and propose the same value $v$, then the consensus will end in the first round.
	%All the processes vote $\mathbb{A}$ for round $0$. 
	%By the validity of BRB, all the processes broadcasting the same value is equivalent to a well-behaved sender broadcasting that value.
	%Then all the processes deliver $\mathbb{A}$ for ballot $\langle 0, \bot \rangle$ and prepare ballot $\langle 1, v \rangle$.
	%They broadcast $\mathbb{C}$ for ballot $\langle 1, v \rangle$ and by validity of BRB, all the processes deliver $\mathbb{C}$ for the same ballot and decide $v$.
	
	
	
	%If all processes are well-behaved and some process decides a value $v$, then before the decision from consensus, $v$ was delivered in a $\mathbb{C}$ message for ballot $b$ by the well-behaved process.
	%Let assume the ballot is $\langle r, v \rangle$.
	%By the integrity of BRB, a well-behaved process broadcast $\mathbb{C}$ for the ballot $\langle r, v \rangle$.
	%A well-behaved process only broadcast $\mathbb{C}$ for its $\candidate$.
	%The $\candidate$ variable is asisgned with two potential values: its own proposal or the $\prepared$ value.
	%If it's the first case, we proved the decision for consensus was proposed by a well-behaved process.
	%If it's the second case, the $\prepared$ variable is updated when a process deliver $\mathbb{A}$ to all the ballots lower and incompatible than $\prepared$.
	%By the integrity of BRB, some well-behaved process broadcasts $\mathbb{A}$ for the ballots lower and incompatible than $\langle r, v \rangle$. 
	%A well-behaved process broadcasts $\false$ only when it proposes a value for consensus or trigger a time out for a round.
	%In the first case, we proved that $v$ was proposed by some well-behaved process.
	%In the second case, the time out is set when a process receives a quorum of messages vote for a round $r' > r$.
	%By induction, the vote was from some well-behaved process's proposal.
\end{proof}

%\xl{We may need to prove a variant of the integrity of BRB: if all the processes are well-behaved and some process deliver a value, the that value was proposed by some process. The proof is the same as BRB's normal integrity, we only need to change the last step that the echo was sent by some well-behaved process.}

%\textbf{Weak liveness}
\begin{lemma}[Termination]
	If the quorum system $\Q$ is strongly available for $P$, then the consensus protocol guarantees termination for $P$.
\end{lemma}

\begin{proof}
	
	%Eventually all the well-behaved processes trust the same well-behaved process.
	%By validity of BRB, the well-behaved leader abort all the previous round and commit its proposal for the strongly available set.
	

	%We assume that eventually all the well-behaved processes propose the same value $v$.
	%Then by the exponential time out, after GST, all the well-behaved processes advance to the same round.
	
	%Then the processes that is strongly available will can abort the
	%Eventually in a round all the well-behaved processes propose the same value.
	%By the validity, totality and consistency of BRB, all the well-behaved processes prepared the value and decide that value. 
\ec{
A process decides a value $v$ when it delivers a ballot $\angled{r,v}$ from a $\mathbb{C}$ broadcast from a leader.
We consider well-behaved and Byzantine leaders separately.
If a well-behaved leader is given a sufficient amount of time, it will eventually broadcast $\mathbb{C}$ $\angled{r,v}$.
This is for two reasons.
Firstly, $v$ is finite and fixed for each well-behaved process.
Secondly, each incremental step (preparing and aborting a ballot) requires a finite amount of time.
Thus, the well-behaved leader, if given sufficient time, will increment from $\angled{r,1}$ through $\angled{r,v-1}$ and eventually reach $\angled{r,v}$, in which they broadcast $\mathbb{C}$.
}

\ec{
For a Byzantine leader, if they broadcast $\mathbb{C}$ $\angled{r,v}$ at any point, we are done.
Otherwise, they can keep preparing and aborting ballots.
However, we will see they cannot do this indefinitely.
}

\ec{
Our leader election abstraction guarantees that eventually a well-behaved process will be elected the leader an infinite amount of times.
A process is elected as a leader for only a finite amount of time $t$.
Whenever leadership is passed from one process to another, $t$ is doubled.
This guarantees us two properties.
Firstly, since $t$ is doubled everytime leadership is passed, a well-behaved process will eventually be given a sufficient amount of time as the leader.
Secondly, since $t$ is finite, a Byzantine leader cannot halt progress indefinitely.
Thus, eventually some leader will broadcast $\mathbb{C}$ for some $\angled{r,v}$.
}

\end{proof}


==> Xtras.tex <==
8. There is no cycle composed only from one-direction edges in the sink component.

8. There is no one-direction edge in the sink component: $\forall p, q \in \mathbf{Sink}$, if $(p, q) \in E$, then $(q, p) \in E$. We can prove this statement by contradiction in all the cases. Let's assume that there is a one direction edge in the sink component: $\exists p, q, \in \mathbf{Sink}$, such that $(p, q) \in E \land (q, p) \notin E$. 

The first case is that there are only two vertices in the sink component. We reach a contradiction. Because the sink component is strongly connected. But there is no path from $q$ to $p$. 

The second case is that there are only three vertices in the sink component. Then we have $(p, q) \in E \land (q, r) \in E \land (r, p) \in E$ because of the existence of one path from $q$ to $p$ with $(q, p) \notin E$. $\{ q \} \notin \mathbf{MQ}$ becasue of $(q, r) \in E$. The same goes for $\{ r\} \notin \mathbf{MQ} \land \{ p \} \notin \mathbf{MQ}$. From statement 5 we have the minimal quorums are in the sink component. Then the minimal quorums contains as least two vertices. From statement 1, we know that minimal quorums are cliques. Then we can only have minimal quorums as $\mathbf{MQ} = \{ \{q, r\}, \{r p\} \}, \mathbf{MQ} = \{ \{q, r\} \} or \mathbf{MQ} = \{ \{r p\} \}$. Without losing of generality, let's assume that $ \{q, r\} \in \mathbf{MQ}$. 
%Then we have $(p, r) \in E$ because of statement 2. 
Since all the quorums contains at least one minimal quorum, we have $\{p, q, r\} \in \mathbf{MVQ}(p)$. Then for vertex $r$, we can have $\{r, p\} \in \mathbf{MVQ}(r)$ or $\{q, r, p\} \in \mathbf{MVQ}(r)$. If $\{r, p\} \in \mathbf{MVQ}(r)$, then we have $\{r, p\} \in \mathbf{MQ}$, which contradict $\{p, q, r\} \in \mathbf{MVQ}(p)$. If $\{q, r, p\} \in \mathbf{MVQ}(r)$, it contradicts with $\{q, r\} \in \mathbf{MQ}$.
%it will contradict $\{p, q, r\} \in \mathbf{MVQ}(p)$

The last case is when there are more than three vertices in the sink component. Because we have $(p, q) \in E \land (q, p) \notin E$ and the sink component is strongly connected. Then there is a path from $q$ to $p$. Let's assume that the last vertex in the path is $s$ and we have $(s, p) \in E$. Because $(p, q) \in E \land (q, p) \notin E$, we have $\exists Q_1 \in \mathbf{MVQ}(p) \land p, q \in Q_1$. And because the edge from $p$ to $q$ is one-direction, we have $\exists Q_3 \subset Q_1 \land p \notin Q_3 \land Q_3 \in \mathbf{MVQ}(q) \land (p, r) \in E$. For vertex $s$, we have $\exists Q_2 \in \mathbf{MVQ}(s) \land p, s \in Q_2$. From quorum intersection property, we have $Q_2 \cap Q_3 \notin \emptyset$. Then we have $\exists r \in Q_2 \cap Q_3, $

How to reduce more than three vertices to the case of three vertices.

One sink in the byzantine quorum graph is the necessary condition for a correct corresponding  byzantine quorum system.

%First of all, the sink component itself is a quorum in the system. Notice that not all strongly connected component is a quorum in the system. The strongly connected component with outgoing edges may not be able to form a complete quorum. Secondly, every quorum in the system contains at least one minimal quorum. If the minimal quorums (top-tires) are not completely inside the sink component, $\exists T \in \Q, T \nsubseteq Sink$, then for all the processes outside of the sink components $ \forall t, t \in T \setminus Sink, \exists s \in Sink, (t, s) \in E, (s, t) \notin E $. This contradicts the statement that minimal quorums are strongly connected subgraphs.

%Statement: the quorum intersection with at least one correct process condition = the sink component after the removal of byzantine processes is still strongly connected. 

This necessary condition can be checked when a process suspect some processes and try to remove them from its own quorums without losing safety property.  

%We prove the equivalence in two directions. 

We prove that the quorum intersection with at least one correct process implies the minimal quorum set is still strongly connected. 

%the sink component after the removal of byzantine process is still strongly connected. $\forall U_1, U_2 \in \mathbf{U}, \forall B \in \mathbf{B}, U_1 \cap U_2 \notin B \implies \forall B \in \mathbf{B}, (Sink \setminus B, E \setminus B )$ is strongly connected. We prove this statement by contradiction. Let's assume that $\exists B \in \mathbf{B}, (Sink \setminus B, E \setminus B)$ is not strongly connected. 

%Then there will be at least two disjoint components and that will produce disjoint minimal quorums, which violates the assumption. 

Maybe useful to add and remove processes while maintaining safety.

The sink component is like the leader?

What does the strongly connected component means? Is it a subset of minimal vertex quorum?

What is the relation between minimal vertex quorums and quorums? The quorum system constructed from minimal vertex quorums with quorum intersection and quorum availability is the necessary and sufficient condition for the original quorum system to hold the same properties.

Necessity: We want to prove that: with a fixed actual Byzantine failure set $B$, we have $\forall Q_1 \in \Q(v), \forall Q_2 \in \Q(v'), Q_1 \cap Q_2 \setminus B \neq \emptyset \wedge \exists v'',  Q_3 \in \Q(v''), Q'' \cap B = \emptyset$, then we can infer $\forall v, v'', \forall Q_1 \in MVQ(v), \forall Q_2 \in MVQ(v'), Q_1 \cap Q_2 \setminus B \neq \emptyset \wedge \exists v'',  Q_3 \in MVQ(v''), Q'' \cap B = \emptyset$. The proof for quorum intersection is straightforward. All the minimal vertex quorums are quorums for some specific nodes, we can directly apply the quorum intersection property for quorums to get the quorum intersection property for minimal vertex quorums. For quorum availability, if we have $ \exists v'',  Q_3 \in \Q(v''), Q'' \cap B = \emptyset$, then acoording to the definition of minimal vertex quorum, either $Q_3 \in MVQ(v'')$ or $\exists Q_4 \subset Q_3, Q_4 \in MVQ(v'')$. Either way there exists a minimal vertex quorum of node $v''$ that does not overlap with $B$. 


==> graph.tex <==
% \section{Topology of Consistent Quorum Systems}
% \section{Topology of Cohesive Quorum Systems}
% \section{Topology of Quorum Systems}
%\section{Graph characterization of Quorum Systems}
\label{sec:graph-and-sink}

\subsection{\textbf{Quorum Graphs}}
% ☞{Presentation: ?}

% ☞{Condition to be made explicit: every minimal quorum is an individual minimal quorum for all its members.}

% ☞{Abstract quorums needed for sink property}
% \xl{Personal quorums instead of abstract quorums, since it does not dependent on the quorum slices concepts}

% ☞{Graph is an over-approximation, the same arcs for all quorums.}


The quorum graph of a quorum system $𝓠$ is
a directed graph $G = (\dom(𝓠), E)$ where
vertices are the domain of $𝓠$, and
$(p, p') ∈ E$ iff $p' ∈ 𝓠(p)$, \ie, $p'$ is a member of an individual minimal quorum for $p$.
% 
Intuitively, the edge $(p, p')$ represents the fact that $p$ directly consults with $p'$.
% 
We refer to a quorum system and its graph characterization interchangeably.
% 
The quorum systems that we consider in this section have quorum intersection and quorum sharing.
We prove the following lemma and theorem of the quorum graph, which will help us find the leader in the sink component in the quorum graph.
% \ml{Slices used next. Needs to be defined.}
    
    
\begin{comment}
        \begin{figure}[H]
            \centering
            ∈cludegraphics[scale = 0.4]{example1.png}
            \caption{Quorum graph for an FBQS. 
                ☞{Update MVQ notation.}
                ☞{To use $𝓠$.}
            }
            \label{fig:eg1}
        \end{figure}
\end{comment}
    
    
\begin{lemma}[]
    \label{lem:well_behaved_MQ_discovery}
    A quorum is a minimal quorum iff it is an individual minimal quorum for all its well-behaved members.
\end{lemma}

This lemma can serve as a proof when a process claims its presence in the minimal quorums.
We later use it in the sink discovery algorithm to produce a proof that can be verified by any process without global quorum system information.
The correctness of the proof variable does not depend on the quorums of Byzantine processes
and it is resilient against the attack that Byzantine processes can lie about their quorums. 

\begin{theorem}[]
	\label{thm:theorem1}
	All well-behaved processes of the minimal quorums are 
	in the sink component of the quorum graph.
\end{theorem}
    
We use this lemma and the sink discovery algoruthm below to find the only sink component of the quorum graph.
The output of the sink component algorithm helps us find the leader which is a well-behaved process in the sink component.

    % \begin{lemma}
        % \label{lem:well_behaved_MQ_discovery}
        % If a quorum is an individual minimal quorum for all its well-behaved processes, 
        % it is a minimal quorum.
        % %     ,
        % %     \ie, $∀q. \ ∀p ∈ q ∩ 𝓦. \ q ∈ 𝓠(p) ⇒ q ∈ MQ(𝓠)$.
        % \end{lemma}
    % 
    % \begin{proof}
        % The proof is by contradiction. 
        % Assume that $q$ is not a minimal quorum.
        % Since $q$ is an individual minimal quorum for $p$ but not a minimal quorum, 
        % there is a minimal quorum $q'$ 
        % % of $p$ 
        % such that 
        % % $p ∈ q'$ and 
        % $q' ⊂ q$.
        % There is a well-behaved process $p$ in $q'$.
        % % (Otherwise, by definition, $q$ is trivially a minimal quorum.)
        % % $\exists q' \subset q, q' \in MQ$. 
        % By \autoref{lem:lemma1},
        % $q'$ is an individual minimal quorum 
        % for all well-behaved processes in $q'$ including $p$.
        % % by %\autoref{lem:well-behaved-self-closed-quorums}
        % % 
        % However, this contradicts with the assumption that
        % $q$ is a individual minimal quorum for $p$
        % and
        % $q' ⊂ q$.
        % % $q' \in \Q(p')$ contradicts with the assumption that $q \in \Q(p')$.
        % % Therefore, we proved that $q$ is a minimal quorum.
        % \end{proof}
    


==> proofs.tex <==
\clearpage
\section*{\textbf{Appendix}}

\section{Graph Characterization and Sink Discovery}

\ml{Everything in this section Cite the PODC submission. Just here to make it self contained.}

\subsection{Graph}

\begin{lemma}[]
	%\label{lem:well_behaved_MQ_discovery}
	A quorum is a minimal quorum iff it is an individual minimal quorum for all its well-behaved members.
\end{lemma}

\begin{proof}
	We first show the only if direction.
	Consider a minimal quorum $q$.
	% We show that
	% $q$ is an individual minimal quorum for
	% every well-behaved member of $q$.
	% \ie,
	% $∀ q ∈ MQ. \ ∀ p ∈ q ∩ 𝓦. \ q ∈ 𝓠(p)$. 
	% 
	% Consider a minimal quorum $q$. 
	% The quorum $q$ must be an individual minimal quorum for some process $p ⃰ ∈ q ∩ 𝓦$.
	% By the quorum subsumption property,
	By the quorum sharing property,
	%of personal quorum system
	all the well-behaved processes in $q$ have an individual minimal quorum $q'$ included in $q$.
	% , \ie,
	% $∀ p ∈ q ∩ 𝓦, ∃ q' ∈ 𝓠(p), q' ⊆ q$.
	% Therefore, 
	Since $q$ is a minimal quorum, $q' = q$.
	% Thus, 
	% $∀ q ∈ MQ. \ ∀ p, p' ∈ 𝓦 ∩ q. \ (p, p') ∈ E$.
	
	
	The proof of the if direction is by contradiction. 
	Assume that $q$ is not a minimal quorum.
	Since $q$ is an individual minimal quorum 
	% for $p$
	but not a minimal quorum, 
	there is a minimal quorum $q'$ 
	% of $p$ 
	such that 
	% $p ∈ q'$ and 
	$q' ⊂ q$.
	There is a well-behaved process $p$ in $q'$.
	% (Otherwise, by definition, $q$ is trivially a minimal quorum.)
	% $\exists q' \subset q, q' \in MQ$. 
	By the only if direction,
	% \autoref{lem:lemma1},
	$q'$ is an individual minimal quorum 
	for all well-behaved processes in $q'$ including $p$.
	% by %\autoref{lem:well-behaved-self-closed-quorums}
	% 
	However, this contradicts with the assumption that
	$q$ is a individual minimal quorum for $p$
	and
	$q' ⊂ q$.
	% $q' \in \Q(p')$ contradicts with the assumption that $q \in \Q(p')$.
	% Therefore, we proved that $q$ is a minimal quorum.
	% 
\end{proof}


\newpageprime
   We remember that a subset of vertices of a graph that are pair-wise connected are a clique.
 % A subset of the vertices of a graph is
 % A clique is 
 % maximal
 % % in a graph 
 % if no proper superset of it is a clique.
 
 \begin{lemma}[]
 	\label{lem:lemma1}
 	Well-behaved processes in a minimal quorum
 	are a clique.
 \end{lemma}
 
 This is immediate from \autoref{lem:well_behaved_MQ_discovery}.
 

 \begin{lemma}[]
 	\label{lem:lemma2}
 	 	Every well-behaved process is adjacent to all processes of at least one minimal quorum.
 \end{lemma}
 
 \begin{proof}
 	By the definition of quorum systems,
 	a process $p$ 
 	has at least one quorum $q$, and
 	is a member of its own quorum $q$.
 	The quorum $q$ contains a minimal quorum $q'$.
	The process $p$ has an edge to every member of $q$ and, thus, $q'$.
 \end{proof}
 

 \begin{lemma}[]
 	\label{lem:lemma3}
	Well-behaved processes in the minimal quorums induce a strongly connected graph.
 \end{lemma}
 
 \begin{proof}
	Consider a pair of minimal quorums $q₁$ and $q₂$, and
	two well-behaved processes $p₁ ∈ q₁$ and $p₂ ∈ q₂$.
	The consistency property states that
 	% for every pair of quorums $q₁$ and $q₂$,
 	there is at least a well-behaved process $p$ in the intersection of $q₁$ and $q₂$.
 	By \autoref{lem:lemma1},
 	the following edges are in the quorum graph:
 	$(p₁, p)$, $(p, p₂)$, $(p₂, p)$ and $(p, p₁)$.
 	Therefore, 
 	$p₁$ and $p₂$
 	are strongly connected.
 \end{proof}
 
 
 We remember that the condensation of a graph is 
 the graph resulted from contracting each of its strongly connected components to a single vertex.
 A condensation graph is a directed acyclic graph (DAG). DAGs have sink and source vertices.
 A component of the graph that is contracted to a sink in the condensed graph is called a sink component.

 \begin{lemma}[]
 	\label{lem:lemma4}
 	All well-behaved processes in minimal quorums are 
	in a sink component of the quorum graph.
 \end{lemma}
 
 \begin{proof}
 	By \autoref{lem:lemma3},
 	the set of minimal quorums is a strongly connected subgraph.
 	Therefore, it falls in a strongly connected component.
 	By \autoref{lem:lemma2},
 	there are edges to this component from the processes of every component.
 	Therefore,
 	this component must be a sink component.
	Otherwise, the sink components will have edges to it 
 	that contradicts the definition of the sink.
 \end{proof}

 \begin{lemma}[]
 	\label{lem:lemma5}
 	There exists a minimal quorum in 

	every sink component of the quorum graph.
 \end{lemma}
 
 \begin{proof}

 	Consider a sink component $S$ of the quorum graph.
 	By \autoref{lem:lemma2},
 	there are edges in the quorum graph
 	from $S$ to
 	all processes of a
 	minimal quorum $q$.
 	This quorum $q$ should be inside $S$.
 	Otherwise,
 	the fact that there are edges from $S$ to $q$
 	contradicts the assumption that $S$ is a sink component.
 \end{proof}

 \begin{lemma}[]
	\label{lem:lemma6}
 	Every quorum graph has only one sink component.
 \end{lemma}
 
 \begin{proof}
 	The proof is by contradiction.
 	If there are two sinks,
	by \autoref{lem:lemma5},
	there is a minimal quorum in each sink.
	By the quorum intersection property,
	the two minimal quorums have an intersection;
	thus, the two sinks have an intersection.
	However, components are disjoint.
 \end{proof}
 
 
 \begin{theorem}[]
 	%\label{thm:theorem1}
 	All well-behaved processes of the minimal quorums are 
 	in the sink component of the quorum graph.
 \end{theorem}
 
 This is straightforward from 
 \autoref{lem:lemma4} and \autoref{lem:lemma6}.
  
 


\clearpageprime
\subsection{Sink Discovery}
\label{sec:discovery}

\begin{algorithm}
	
	\caption{Sink Discovery Protocol}
	\label{alg:discovery}
	\DontPrintSemicolon
	\SetKwBlock{When}{when received}{end}
	\SetKwBlock{Upon}{upon}{end}
	
	\textbf{Variables:}  \;
	\ \ \ $Q$ \Comment{The individual minimal quorums of $\self$} \;
	\ \ \ $\mathit{qmap} : 𝓟 \mapsto \mathsf{Set[2^𝓟]}$\;	    
	\ \ \ $\insink : \mathsf{Boolean} ←\false$ \;
	\ \ \  $F : 2^𝓟$ \;
	% 	\ \ \ $\mathit{qmap} : \cup Q \mapsto \mathsf{Set[𝓟]}$\;	
	 \ \ \ $\proofLE : \mathsf{Set}[\text{Exchange or Extend messages}]$\;	
	
	\Uses $\colon$ \;
	\ \ \ $\apl : 𝓟 ↦ \mathsf{AuthPerfectPointToPointLink}$ \;
	
	\Upon ($\request \ \Discover$\label{algD:discover-handler}){    % for $p \in 𝓟$
		% 		$\apl(p) \ \request \ \Exchange(Q)^\mathit{sig}$ \mbox{ for each} $p ∈ \cup Q$ \label{algD:exchangeSend}\;
		$\apl(p) \ \request \ \Exchange(Q)$ \mbox{ for each} $p ∈ \cup Q$ \label{algD:exchangeSend}\;
	}
	
	% 	\Upon ($\response$ \mbox{$\apl (p)$}, \mbox{$\Exchange(Q')^{σ}$} \label{algD:UponCondInSink} ){
		\Upon ($\response$ \mbox{$\apl (p)$}, \mbox{$\Exchange(Q')$} \label{algD:UponCondInSink} ){
			$F ← F \cup \{p\}$ \label{algD:update-follower} \;
			% 		$\mathit{qmap}(p) ← Q'^{σ}$
			$\mathit{qmap}(p) ← Q'$
		}
		
		\Upon($\exists q \in Q. \ \forall p \in q. \ q \in$ \mbox{$\mathit{qmap}(p)$ \label{algD:mqDiscovery}}){
			$\insink \leftarrow \true$ \label{algD:insink0} \;
			$\proofLE[q] \leftarrow  \mathit{qmap} |_q$ \;
			$\apl(p) \ \request \ \Extend(q)$ \mbox{ for each} $p∈ \cup Q$ \label{algD:extendSend} \;
			% 		$\apl(p) \ \request \ \Extend(q, \mathit{qmap} |_q)$ \mbox{ for each} $p∈ \cup Q$ \label{algD:extendSend} \;
		}
		
		% 	\Upon($\response$ $\overline{\mbox{$\apl(p')$}}, \Extend\mbox{$(q', \mathit{qs})$}$ 
		% 	\Upon($\response$ $\overline{\mbox{$\apl(p')$}}, \Extend\mbox{$(q')$}$ 
		\Upon($\response$ $\overline{\mbox{$\apl(p)$}}, \Extend\mbox{$(q)$}$ 
		% 	$\mbox{such that}$ 
		$\mbox{s.t.}$ 
		% 	$p' ∈ \mathsf{dom}\mbox{$(\mathit{qs})$}$ 
		% 	$∃q ∈ Q. \ \{ \overline{p'} \}$ $=$ $\mathsf{dom}\mbox{$(\mathit{qs}) ∩ q$}$
		$∃q' ∈ Q. \ \{ \overline{p} \}$ $=$ $q ∩ q'$
		 	\ $∧$ \ $\mathit{validq}\mbox{$(q)$}$
		\label{algD:extendReceived}\label{algD:cond}){  
			% 		\If{$\mathit{proof'}$ is valid}{
				%         $\textbf{let} \ q ← \mathit{dom}(\mathit{quorums'}) \ \textbf{in}$ \;
				%         $\textbf{let} \ \{ \overline{p ↦ Qₚ_{_σₚ}} \} ← \mathit{quorums'} \ \textbf{in}$ \;
				%         $\textbf{let} \ q' ≔ \mathit{dom}(qs) \ \textbf{in}$ \;
				%         $\textbf{let} \ \{ \overline{p ↦ Qₚ} \} ≔ \mathit{qs} \ \textbf{in}$ \;
				%         $\textbf{let} \ q = \{ \overline{p} \} \ \textbf{in}$ \;
				% 		\If{$\forall p \in q. \ q \in \mbox{$\mathit{quorums'}(p)$}$ }{
					% 		\If {$($\mbox{for each} $p$, $q' \in Qₚ ∧ \mbox{$\mathit{athenticate}(σ, p))$}$ $∧$ 
						%\If {
							 		%\textcolor{blue}{
								 		%$\mathit{validq}\mbox{$(q')$}$\label{algD:cond}}{
								$\insink \leftarrow \true$ \label{algD:insink1} \;
								$\proofLE[q] \leftarrow \overline{\apl(p)}, \Extend(q)$ \;
								%}
						}
					\end{algorithm}
							
% \newpageprime

% In the previous section,
% we saw that
% any change outside of the sink component of a quorum graph
% does not affect quorum intersection.
% 
% 
In this section, we see a decentralized protocol
that can find whether each process is in the sink component of the quorum graph.
We first see the protocol and then its completeness and accuracy
guarantees.


\textbf{∗Protocol. \ }
Consider a quorum system 
with quorum intersection, sharing and availability.
The sink discovery protocol in
\autoref{alg:discovery} 
finds whether 
each well-behaved process is in the sink.
It also finds the set of its followers.
(A process $p$ is a follower of process $p'$ iff $p$ has a quorum that includes $p'$.)
% 
The protocol has two phases.
In the first phase, it finds the well-behaved minimal quorums,
\ie, every minimal quorum that is a subset of well-behaved processes.
Since well-behaved minimal quorums are inside the sink,
the second phase extends the discovery from 
processes found in the first phase to 
other processes in the same strongly connected component.
% 
% The sink component is strongly connected despite Byzantine processes.


% Because all the members of this quorum are well-behaved, we can find this quorum by exchanging quorum information with neighbors.



\textit{Variables and sub-protocols.\ } 
%
In the quorum system $𝓠$,
each process $\self$ stores 
its own set of individual minimal quorums $Q=𝓠(\self)$,
a map $\mathit{qmap}$ from other processes to their quorums
which is populated as processes communicate,
% and
the $\insink$ boolean that stores whether the process is in the sink, 
and
the set of follower processes $F$.
% The latter two are set by the protocol.
% 
% 
% 
% 
% 
The protocol uses 
authenticated point-to-point links $\apl$.
% 
% The authenticated point-to-point link $\apl$
They
% ensures that
provide
the following safety and liveness properties.
% for well-behaved processes.
% Validity: Termination:
If the sender and receiver are both well-behaved, 
then the message will be eventually delivered. 
% 
Every message that a well-behaved process delivers from a well-behaved process is sent by the later, \ie, 
the identity of a well-behaved process cannot be forged.
% 
% The well-behaved sender's identity can be verified by it's signature and can not be forged by Byzantine processes. 



\textit{Protocol.\ } 
% 
When processes receive a $\Discover$ request
(at \autoref{algD:discover-handler}),
they exchange their quorums with each other.
In this first phase,
each process sends an $\Exchange$ message with its quorums $Q$ 
% and signature $\mathit{sig}$
to all processes in its quorums.
% (at \autoref{algD:exchangeSend}).
% 
When a process receives an $\Exchange$ message
(at \autoref{algD:UponCondInSink}),
it adds the sender to the follower set $F$,
and stores the received quorums 
% and signature 
in its $\mathit{qmap}$.
% 
As $\mathit{qmap}$ is populated,
when a process finds that one of its quorums $q$ is a quorum of every other process in it as well
(at \autoref{algD:mqDiscovery}),
by \autoref{lem:well_behaved_MQ_discovery} and \autoref{thm:theorem1},
it finds itself in the sink.
Thus, it
sets its $\insink$ variable to $\true$
in the first phase
(at \autoref{algD:insink0}).
% 
% As we will see,
The processes of every well-behaved minimal quorum are found in this phase.
The process then sends an $\Extend$ message with the quorum $q$ 
% and the signatures of the members of $q$
to all processes of its own quorums $Q$.
% (The projection $\mathit{qmap} |_q$ restricts the domain of $\mathit{qmap}$ to the set $q$.)
The $\Extend$ messages are processed in the second phase.
% This starts the second phase.




The processes $P₁$ of every well-behaved minimal quorum find themselves to be in the sink in the first phase.
Let $P₂$ be the well-behaved processes of the remaining minimal quorums.
A pair of minimal quorums have at least a well-behaved process in their intersection.
Therefore,
every 
% well-behaved 
process in $P₂$
% of the remaining minimal quorums
is a neighbor of a process in $P₁$.
% a process that found itself in the sink in the first phase.
% 
Thus, 
in the second phase,
the processes $P₁$
% the processes that found themselves in the sink in the first phase
can send $\Extend$ messages to processes in $P₂$, and 
% make
inform
them
% the 
% % well-behaved 
% processes 
% in $P₂$
% of the remaining minimal quorums 
% find 
that they are in the sink.
% 
% 
% Case 2:
% q' has one Byzantine p, and p obtains qs
% intersection prevents p from making others outside the sink think they are in the sink.
% This can be with more Byzantine processes in addition to p.
% 
% Therefore,
The protocol lets a process receive an $\Extend$ message containing a quorum $q$ 
only when the same message comes from 
the intersection 
% a set of processes 
% $P' = \{ \overline{p'} \}$ 
of $q$ 
and 
one of its own quorums $q'$
(at \autoref{algD:extendReceived}).
% 
Let us see why a process in $P₂$ 
cannot accept an $\Extend$ message from a single process.
% these conditions are needed.
A minimal quorum $q$ that is found in phase 1 can have a Byzantine process $p₁$.
The process $p₁$ can send an $\Extend$ message to a process $p₂$
even if $p₂$ is not a neighbor of $p₁$,
% even if $p'$ is not in the quorums of $p$,
% 
% outside the sink 
and make $p₂$ believe that it is in the sink.
% 
Therefore, a process $p₂$ in $P₂$ needs to receive the message from an intersection 
of $q$ and one of its own quorums.
% Since there is at least one well-behaved process $p$ in the intersection.
% Byzantine processes cannot single-handedly mislead
% Receiving the same message from the intersection,
Since there is a well-behaved process $p₁$ in the intersection of 
the two 
% every pair of 
quorums,
the process $p₂$ can then trust the $\Extend$ message.
% 
%
% 
% It further 
% authenticates the signatures accompanying $q'$
% to make sure that 
% $q'$ is an individual minimal quorum for all its members
% (at \autoref{algD:cond}).
%
% When the checks pass,
When the check passes,
the receiving process finds itself to be in the sink,
and 
sets the $\insink$ variable to $\true$
in the second phase
(at \autoref{algD:insink1}).



Let $\ProtoSink$ denote 
the set of well-behaved processes where the protocol sets the $\insink$ variable to $\true$.
% Before considering the guarantees of the protocol,
% we first see a general property of quorum systems.
% We now consider the guarantees of the protocol.
% 
% 
%
% 
\newpageprime
% \textbf{∗Completeness. \ }
% 
The discovery protocol is complete:
% Our sink discovery function is complete but not accurate:
all the well-behaved processes of minimal quorums will eventually know that they are in the sink
(\ie, set their $\insink$ variable to $\true$).
% But the sink component can also include some Byzantine processes.
% 

% 
% The above lemma
% % immediately results in the following corollary.
% immediately 
% that results in the following lemma.


% ☞{Completeness for for members of every well-behaved minimal quorum for the 1st phase}
% The $\Exchange$ phase of the sink discovery protocol is complete: 


% \begin{lemma}[Completeness for Phase 1]
	% % \begin{lemma}[Correctness for Phase 1]
		% % \begin{lemma}[Validity for Phase 1]
			% 	\label{lem:exchange_complete}
			% \input{ProtoSink1Completeness}
			% \end{lemma}
		% 
		% \inputprime{ProtoSink1CompletenessProof}
		
		
		% ☞{Completeness for all the well-behaved processes in the minimal quorums}
		
		% The $\Extend$ phase of the sink discovery protocol is complete
		% We now consider completeness for phase 2.
		% The $\Extend$ phase of the sink discovery protocol is complete
		
		% \begin{lemma}[Completeness for Phase 2]
			% % \begin{lemma}[Correctness for Phase 2]
				% % \begin{lemma}[Validity for Phase 2]
					% \label{lem:extend_complete}
					% \input{ProtoSink2Completeness}
					% \end{lemma}
				% 
				% \inputprime{ProtoSink2CompletenessProof}
				
				
				% ☞{Properties for the whole protocol}
				
				% \begin{corollary}[Accuracy]
					%     $\ProtoSink ⊆ \Sink$
					% \end{corollary}
				% 
				% This is immediate from \autoref{lem:acc-1} and \autoref{lem:acc-2}.
				
				% % This is immediate from \autoref{lem:exchange_complete} and \autoref{lem:extend_complete}.
				% % \autoref{lem:exchange_complete} and \autoref{lem:extend_complete}
				% The above lemma
				% % immediately results in the following corollary.
				% immediately results in the following lemma.
				% % The above two lemmas
				% % immediately result in the following corollary.
				
				
% \begin{corollary}[Completeness]
\begin{lemma}[Completeness]
	\label{cor:completenss-discovery}
	% \begin{corollary}[Validity]
		% Eventually $(∪ MQ(𝓠)) ∩ 𝓦 ⊆ \ProtoSink$.
		Forall $q ∈ MQ(𝓠)$, eventually $q ∩ 𝓦 ⊆ \ProtoSink$.
		% Well-behaved processes of 
		% % in the 
		% minimal quorums will eventually be in $\ProtoSink$.
		%     \ie,
		% %     Well-behaved minimal quorums will be eventually in $\ProtoSink$, \ie,    
		%     $∀q ∈ MQ(𝓠), p.$ 
		% %     \ 
		%     if
		%     $p ∈ q ∩ 𝓦$
		%     then eventually
		%     $p ∈ \ProtoSink$.
\end{lemma}
We prove both the completeness and accuracy of the two phases in turn.
	% 
The accuracy property states that $\ProtoSink$ is a subset of the sink component.

						

% \subsection{\textbf{Sink Discovery, Completeness 1}}
% \textbf{Sink Discovery, Completeness}
\subsection{Sink Discovery, Completeness}
Let the set $\ProtoSink$ partition into
$\ProtoSink₁$ and $\ProtoSink₂$ that denote
the set of well-behaved processes at which the protocol sets the $\insink$ variable to $\true$
in phase 1 (at \autoref{algD:insink0}),
and 
in phase 2 (at \autoref{algD:insink1})
respectively.


% \textbf{\autoref{lem:exchange_complete}}.
\begin{lemma}[Completeness for Phase 1]
    % \begin{lemma}[Correctness for Phase 1]
        % \begin{lemma}[Validity for Phase 1]
            \label{lem:exchange_complete}
            \textit{\input{ProtoSink1Completeness}}
        \end{lemma}
        \input{ProtoSink1CompletenessProof}
        
        \newpageapp
        
        % \subsection{\textbf{Sink Discovery, Completeness 2}}
        \begin{lemma}[Completeness for Phase 2]
            % \begin{lemma}[Correctness for Phase 2]
                % \begin{lemma}[Validity for Phase 2]
                    \label{lem:extend_complete}
                    % \textbf{\autoref{lem:extend_complete}}.
                    \textit{\input{ProtoSink2Completeness}}
                \end{lemma}
                
                \input{ProtoSink2CompletenessProof}
                
                \newpageapp
                
                
                
                % \subsection{\textbf{Sink Discovery, Accuracy 1}}
                \subsection{\textbf{Sink Discovery, Accuracy}}
                A group of Byzantine processes fake to be a quorum
                and send an $\Extend$ message to make a process that 
                is outside the sink
                believe that it is in the sink.
                This can violate accuracy.
                Therefore, 
                a check $\mathit{validq}$ is needed to ensure that 
                the processes in $q$ can form a valid quorum in the system
                (at \autoref{algD:cond}).
                For example, 
                the heterogeneous quorum systems of
                both Stellar \cite{lokhava2019fast} and Ripple \cite{schwartz2014ripple}
                use 
                hierarchies of processes
                and
                size thresholds 
                to recognize quorums.
                In the appendix, we prove the accuracy of the two phases in turn that results in the following lemma. 
                % \textbf{\autoref{lem:acc-1}}.
                \begin{lemma}[Accuracy of Phase 1]
                    \label{lem:acc-1}
                    \textit{\input{ProtoSink1Accuracy}}
                \end{lemma}
                
                \input{ProtoSink1AccuracyProof}
                
                \newpageapp
                
                % \subsection{\textbf{Sink Discovery, Accuracy 2}}
                % \textbf{\autoref{lem:acc-2}}.
                \begin{lemma}[Accuracy for Phase 2]
                    \label{lem:acc-2}
                    \textit{\input{ProtoSink2Accuracy}}
                \end{lemma}
                
                \input{ProtoSink2AccuracyProof}
                
\subsection{Sink Discovery, Output variables}

We prove that the correctness of outputs from sink discovery protocol.

\begin{lemma}[Completeness for follwer set]
	\label{lem:follower-completeness}
	Let $\mathit{ProtoF}$ be the follower set by the sink discovery protocol.
	For every well-behaved process, eventually $F \cap \W \mathit{ProtoF}$.
\end{lemma}

\begin{proof}
	Let $p$ and $p'$ be two well-behaved process. 
	If process $p$ is a follower of process $p'$, then by \todo the definition of follower set, $p'$ is in one of $p$'s individual minimal quorum: $\exists q \in \Q(p), p' \in q$. 
	$p$ sends out $\Exchange$ to its quorum members at \autoref{algD:exchangeSend}, which includes $p'$.
	$\Exchange$ messages between two well-behaved processes will be eventually delivered at 
	\autoref{algD:UponCondInSink}.
	Then follower varaible at $p'$ is updates at \autoref{algD:update-follower} to include $p$.
	We proved that the well-behaved followers of a process are eventually included in its $\mathit{ProtoF}$.
	
\end{proof}

\begin{lemma}[Accuracy for in-sink proof]
	\label{lem:proof-accuracy}
	
\end{lemma}



